Comprehensible Artificial Intelligence on Knowledge Graphs: A survey

Artificial Intelligence applications gradually move outside the safe walls of research labs and invade our daily lives. This is also true for Machine Learning methods on Knowledge Graphs, which has led to a steady increase in their application since the beginning of the 21st century. However, in many applications, users require an explanation of the Artificial Intelligences decision. This led to increased demand for Comprehensible Artificial Intelligence. Knowledge Graphs epitomize fertile soil for Comprehensible Artificial Intelligence, due to their ability to display connected data, i.e. knowledge, in a human- as well as machine-readable way. This survey gives a short history to Comprehensible Artificial Intelligence on Knowledge Graphs. Furthermore, we contribute by arguing that the concept Explainable Artificial Intelligence is overloaded and overlapping with Interpretable Machine Learning. By introducing the parent concept Comprehensible Artificial Intelligence, we provide a clear-cut distinction of both concepts while accounting for their similarities. Thus, we provide in this survey a case for Comprehensible Artificial Intelligence on Knowledge Graphs consisting of Interpretable Machine Learning on Knowledge Graphs and Explainable Artificial Intelligence on Knowledge Graphs. This leads to the introduction of a novel taxonomy for Comprehensible Artificial Intelligence on Knowledge Graphs. In addition, a comprehensive overview of the research on Comprehensible Artificial Intelligence on Knowledge Graphs is presented and put into the context of the taxonomy. Finally, research gaps in the field of Comprehensible Artificial Intelligence on Knowledge Graphs are identified for future research.

==> figures/colour_codes.tex <==
% Hier die Hash-codes der BMW Farben:
bmw_color = '#035970'
petrol = '#004750'
light_blue = '#04829B'
blue = '#035970'
dark_blue = '#173B68'
green = '#508130'
red = '#B11926'
orange = '#E96D0C'
yellow = '#FAD022'
dark_grey = '#382E2C'
grey = '#494949'
lighter_grey = '#6F6F6F'
light_grey = '#A8A8A7'
darker_blue = '#0083C6'
lighter_blue = '#468AC9'
berry = '#69103B'
pink = '#8D1E77'
light_pink = '#A33C8D'
purple = '#4B277B'
light_purple = '#794694'

% Hier die Reihenfolge in der die Farben verwendet werden:
# Create bmw colors as matplolib colormap.
colors = (bmw_color, green, yellow, petrol, light_blue, darker_blue, berry,               orange, red, pink, light_pink, lighter_blue, blue , dark_blue,
            purple, light_purple, light_grey, lighter_grey, dark_grey, grey)
bmw_colors = LinearSegmentedColormap.from_list("bmw_colormap", colors)

==> sections/comprehensible_ai.tex <==
%-------------------------------------------
\section{\acs{kg}s for \acs{cai}}\label{sec:kg_for_cai}
%-------------------------------------------
%-------------------------------------------
%--Christoph-- -READY FOR REVIEW-
% Story warum das mittlerweile so ein hype thema ist 
%\ac{ai} applications gradually move outside the safe walls of research labs and invade our daily lives. Many real-world \ac{ai} applications, like in medicine \citep{Bruckert2020} and autonomous driving \citep{Wehner2022}, are safety-critical. Thus, \ac{ai} algorithms used in those fields are regulated \citep{eu2021}. Those regulations give the user of an \ac{ai} system the right to be able to comprehend the \ac{ai}s decision \citep{eu2021}. However, most state-of-the-art \ac{ai} approaches like deep neural networks are too complex and complicated to comprehend for a human observer. Such models are called block box models. This led to increased demand for comprehensible \ac{ai} research in the last years \citep{Schwalbe2021, Futia2020}. 
% TODO:in die einleitung
% KGs sind semantische "powerhouses". diese semantik kann ausgenutzt werden, um erklärungen einer vorhersage/klassifikation etc zu generieren. \citet{Amato2022}
%\acp{kg} in a graph and symbolic representation are inherently comprehensible to a human observer. In addition, \acp{kg} store data in a highly relational manner. This way, every piece of data is embedded in a semantic context. The comprehensible semantic context provided by a \ac{kg} seems promising to explain black boxes \citep{Dragoni2022, Amato2022, Gaur2021}. Furthermore, \acp{kg} give rise to comprehensible algorithms that combine symbolic and sub-symbolic \ac{ai} methods \citep{Amato2022}. That line of research is called the third wave of \ac{ai} \citep{Schmid2021b, Garcez2020}. 
Comprehensible and explainable \ac{ai} as well as \acs{iml} are not sharply defined concepts. This survey follows the understanding of the concepts as introduced in work by \citet{Rudin2019} and \citet{Schmid2021a}. The concepts comprehensible, explainable and interpretable \ac{ai} shall be outlined in the following subsections. 

\subsection{\acs{cai}}\label{sub:comp}
%----Christoph ----------READY FOR REVIEW-
\acs{cai} is about opening up black box models and explaining their input, their inside reasoning and processing, and output in an adequate manner to the relevant stakeholders. 
\acs{cai} makes a black box \ac{ai} model transparent without decreasing its performance. 
Another side of \acs{cai} is developing algorithms that produce explainable \ac{ai} models, so-called white-box models. 
Those white-box models are supposed to perform close to the state-of-the-art \citep{Adadi2018}.

\acs{cai} serves the following four reasons. 
(1) The \acs{cai} model is supposed to justify its judgment and show if the judgment is ethical in a predominant moral system \citep{Adadi2018, Lipton2018}.
(2) Furthermore, explanations help to identify risks and flaws of an \ac{ai} model.
A possible risk is the \emph{Clever Hans} phenomena described by \citet{Lapuschkin2019}. They describe an image classifier that can only classify horses as horses because all pictures with horses had a particular watermark on them. The explanation of the classifier uncovered this flaw \citep{Adadi2018, Lipton2018}. 
(3) That enables researchers or developers to debug and improve the model \citep{Adadi2018, Lipton2018}.
(4) In addition, producing explanations for an \ac{ai} model might uncover unknown rules discovered by the \ac{ai} model \citep{Adadi2018, Lipton2018}.
% Was hälst du von der Figure um den USP unseres Papers nochmal herauszuarbeiten? Dieses Framework haben ja die anderen KG Surveys nicht.
Figure~\ref{fig:cai} displays the generic \ac{cai} framework separating \ac{xai} from \ac{iml}.

\begin{figure}[!ht]
  \centering
  \includegraphics[scale=0.5]{figures/cai_iml_xai.png}
  \caption{Generic \ac{cai} framework separating \ac{xai} from \ac{iml}.}\label{fig:cai}
\end{figure}

%-------------------------------------------
\subsubsection*{\acs{iml}}
\label{subsubsec:iml}
%----Simon 14.04.22 ---------READY FOR REVIEW-
Frequently, \emph{interpretability} in \ac{ml} is achieved by producing statistical explanations that are assumed to be easily understandable by humans and that are added to black box \ac{ml} models. Now, authors argue that truly interpretable \ac{ai} models would require a 
%specific interpretable design 
per default completely human-understandable decision-making processes
to integrate the user into the system to generate interpretability, rather than offering him a set of descriptive tools \citep{Lahav2018, molnar2022}. Such systems, shall, for the scope of this survey, be referred to as \ac{iml} systems. Notably, \ac{iml} focuses on the specific \ac{ml} model that is a per default human-interpretable inference process.% (e.g. by interpreting underlying rules of the model)
\ac{xai} will be outlined in the following.
%, which epitomizes a contrast to other concepts like \ac{xai}, and will be outlined in the following.

%-------------------------------------------
\subsubsection*{\acs{xai}}
%----Christoph Open for Review ---------
% unsere definition 
%\acs{xai} is not a sharply defined concept. Many researchers use it synonymous with interpretability and comprehensibility \citep{Adadi2018}. 
While \acs{iml} tries to uncover the whole decision-making process of the machine learning algorithm, \acs{xai} is about mapping the input of a black box model to its corresponding output. 
That way, \acs{xai} methods provide an explanation of the machine learning model’s behaviour. The inside reasoning and processing of the black box model shall not be made transparent.

A common theme in \acs{xai} is the attribution of a feature by an impact value. The attribution tells how important a feature is for or against a classification. Such methods are so-called attribution methods \citep{Zhou2021, Zhai2006, Bach2015, Ribeiro2016, Lundberg2017}. 
%Attribution methods can be further divided into back-propagation methods\citep{Zhai2006, Bach2015} %like saliency maps \citep{Zhai2006} or \emph{LRP} \citep{Bach2015} 
%and perturbation methods \citep{Ribeiro2016, Lundberg2017}. % like \emph{LIME} \citep{Ribeiro2016} or \emph{SHAP} \citep{Lundberg2017}.
Many other innovative themes exist in \acs{xai},
like counterfactual explanations \citep{Verma2020} or Inductive logic programming (\emph{ILP}) based methods \citep{Rabold2018}.

% TODO: Bezug auf KGs herstellen
%-------------------------------------------
\subsection{\acs{iml} on \acs{kg}s}
\ac{iml} algorithms on \acp{kg} come in many shapes and colors. As argued in subsection \ref{subsubsec:iml}, the main commonality of such models is that they are self-explanatory white-box models for prediction and classification tasks on \acp{kg}. This survey identifies several lines of research in the field of \ac{iml} on \acp{kg}. 
One of the earliest lines of research are Rule Mining algorithms. 

%rule based line of research 
\subsubsection{Rule Mining Approaches to Interpretable Machine Learning on Knowledge Graphs}
One may trace back the roots of rule mining algorithms on \acp{kg} to Inductive logic programming (\emph{ILP}) \citep{Muggleton1991} algorithms like \emph{FOIL} \citep{Quinlan1990}. However, their scope is learning rules from any logical knowledge base, not particular \acp{kg}, and they suffer from scalability issues when it comes to midsized and large \acp{kg} \citep{Cohen1995,Svatek2006,Lao2011}. 

%TODO: FIGURE on how interpretable model looks like. 
One of the first and most impactful white-box rule mining algorithms specifically designed for \acp{kg} was \emph{PRA} \citep{Lao2011}. \emph{PRA} samples numerous path types. Next, random walks through the KG are conducted. The random walks are constrained to follow one of the previously sampled path types. The random walks count the frequency of two nodes being the start and end of the same path type. Finally, the frequencies of possible path types over the nodes are matched via logistic regression. That way, general rules are inferred, and missing links between nodes are predicted. Furthermore, the path types frequencies might be used as the embedding of a node \citep{Lao2011}.
While \emph{PRA} has increased scalability, random walks are still computationally expensive. In addition, the link prediction accuracy is not state-of-the-art since factorization and translation methods, like \emph{RESCAL} \citep{Nickel2011} and \emph{TransE} \citep{Bordes2013}, were introduced. Research following \emph{PRA}, like \emph{SWARM} \citep{Barati2016}, \emph{RBvLR} \citep{Omran2018}, \emph{RDF2rules} \citep{Wang2015}, and \emph{AIME+} \citep{Galarraga2015} on rule-based algorithms addresses those issues. In particular, \emph{AIME+} is another \emph{ILP}-inspired algorithm for scalable rule mining and link prediction on \acp{kg}. \emph{AIME+} builds rules for link prediction by iteratively adding new clauses to a rule such that the approximated coverage and confidence of the new rule is maximized given the \ac{kg} \citep{Galarraga2015}. 
\emph{AIME+} improved on scalability and predictive performance compared to \emph{PRA}. However, modern large-scale \acp{kg} are still out of reach for \emph{AIME+}. 
Ontology Pathfinding (\emph{OP}) \citep{Chen2016a}, also known as \emph{ScaLeKB} \citep{Chen2016b}, scales the idea of \emph{AIME+} to large benchmark \acp{kg} datasets like Freebase. It does so by parallelizing join queries, breaking the rule mining task into smaller sub-tasks, and eliminating unsound and resource-consuming rules before extending them.
In addition, \emph{AnyBLUR} \citep{Meilicke2019} and subsequently \emph{SAFRAN} \citep{Ott2020} build on \emph{PRA} to increase its scalability by an anytime bottom-up technique for rule learning \citep{Meilicke2019} and aggregating rules through a scalable clustering algorithm \citep{Ott2020}. 

The latter rule mining approaches focus on a symbolic representation of the knowledge graph. However, methods relying on symbolic representation suffer from scalability issues while being highly interpretable. In contrast, methods relying on sub-symbolic representation are highly scalable, but interpretability is hard to achieve. 
The following approaches use both types of representation to establish scalable and interpretable machine learning methods on \acp{kg}. 
For example, \emph{NeuralLP} \citep{Yang2017} mines interpretable rules from \acp{kg}. \emph{NeuralLP} is inspired by the probabilistic deductive database \emph{TensorLog} \citep{Cohen2017}. \emph{NeuralLP} learns weighted chain-like logical rules. Those link the head of a query to its tail. It does so by embedding relations in an end-to-end differentiable model as operators. A recurrent neural network learns how to decompose these operators, such as the loss of the link prediction task is optimized \citep{Yang2017}. 
\emph{DRUM} \citep{Sadeghian2019} builds on the idea of \emph{NeuralLP}. It increases the expressivity of \emph{NeuralLP} by an improved representation of the differentiable operators. This allows for learning rules that cover a higher number of relations than \emph{NeuralLP}. Furthermore, it uses a bidirectional recurrent neural network \emph{RNN} to optimize the operators. The bidirectional \emph{RNN} captures information about the backward and forward order in which the relations can appear in the rule \citep{Sadeghian2019}. \citet{Sadeghian2019} show that \emph{DRUM} outperforms state-of-the-art link prediction models like \emph{MINERVA} \citep{Das2017} and \emph{RotatE} \citep{Sun2019} on the inductive link prediction task. 
\emph{RuLES} \citep{Ho2018} is also a neuro-symbolic approach to rule mining. It learns rules guided by a knowledge graph embedding. At each iteration, \emph{RuLES} expands existing rules such that the link prediction performance is optimized. The knowledge graph embedding provides the probability of a rule to be expanded by an atom \citep{Ho2018}. That way, the search space for new rules is pruned, which increases the scalability \emph{RuLES} compared to other rule-mining methods. 

\subsubsection{Pathfinding Approaches to Interpretable Machine Learning on Knowledge Graphs}
%TODO: FIGURE on how interpretable model looks like. 
The latter method's mine interpretable rules from \acp{kg}, which then are used to predict missing links between entities. This approach is straightforward in discovering knowledge and building white box AI models to predict missing links in the \ac{kg}. However, another way of solving the link prediction task is to treat it as a pathfinding problem from the head entity to the tail entity through the KG given the missing relationship. 
\emph{DeepPath} \citep{Xiong2017} builds the fundaments of those methods. It uses \emph{TransE} \citep{Bordes2013} to predict the tail for a head-relationship pair. Next, \citet{Xiong2017} train a reinforcement learning agent to find the most informative path linking the head and tail entity for the predicted triple. However, as the pathfinding is decoupled from the actual link prediction process, the faithfulness required for an explanation method is not given in the case of \emph{DeepPath} \citep{Xiong2017}. 
The method inspired research on interpretable link prediction from the perspective of a pathfinding problem, solved by a reinforcement learner. 
The first method deploying this perspective was \emph{MINERVA} \citep{Das2017}. \emph{MINERVA} models the prediction task of the tail entity given a head entity and a missing relation as a pathfinding problem. \ac{kg} nodes are treated as states, and relations are the actions or paths to transition from one state to the other. A RL agent is trained to walk the optimal path through the \ac{kg} to the correct tail entity. The policy network of the RL agent is an LSTM \citep{Hochreiter1997}. This allows the agent to consider the already walked path whenever picking an action in a state. The agent is rewarded with the value one whenever the agent walks to the correct tail entity. If the agent gets lost, it is rewarded with the value 0 \citep{Das2017}. 
\citet{Lin2018} observe that in an incomplete \ac{kg} the RL agent receives low-quality rewards by false negatives in the training data. This reduces the generalization capacity of the agent at test time. In addition, \emph{MINERVA} provides no optimal paths to the agent at training time. Thus, paths can be learned that accidentally lead to the correct answer. They address this problem by introducing a pre-trained one-hop embedding model, like \emph{ComplEx} \citep{Trouillon2016} or \emph{ConvE} \citep{Dettmers2018} to estimate the reward of unobserved facts. \citet{Lin2018} show that this reduces the impact of false negatives in the training data.\footnote{\emph{MINERVA} adopts the idea of estimating the reward of unobserved facts in an improved version published in 2018 \citep{Das2018}.} Furthermore, \citet{Lin2018} force the agent to explore a diverse set of paths by applying randomly generated edge masks to the KG environment at training time. 
\citet{Bhowmik2020} extend the pathfinding approach to the inductive link prediction domain. This allows link prediction for previously unseen entities. They achieve this by using a graph attention network for policy selection of the reinforcement learning agent and a pre-trained \emph{ConvE} \citep{Dettmers2018} embedding as a reward estimator whenever the predicted link is not in the training set \citep{Bhowmik2020}.
The pathfinding approach to link prediction is also applied to recommender systems. The task here is given a knowledge graph, a user, and a recommendation set of items to find reasoning paths such that the user is connected to each item in the recommendation set \citep{Xian2019, Zhang2020, Zhu2021}. 
In particular, \emph{LOGER} \citep{Zhu2021} deploys a \emph{Markov Logic Network} \citep{Qu2019} to guide the RL agent to the optimal result. The \emph{Markov Logic Network} learns personalized importance scores over paths from the user to recommendation items. To do so, the \emph{Markov Logic Network} learns from previous user behaviour. Next, a RL agent finds the optimal path from the user to the recommendation item by optimizing the correctness of the recommendation and the importance scores of a path \citep{Zhu2021}. 

\subsubsection{Embedding-based Approaches to Interpretable Machine Learning on Knowledge Graphs}
Standard embedding methods show high predictive performance. However, they are not interpretable. A recent line of research tries to mitigate this issue by designing interpretable embedding models. 
%One of the first approaches to this task was by \citet{Abdollahi2016a}. They optimize a matrix factorization for recommending the top explainable items. Explainable items in the authors' notion are items other similar users bought \citep{Abdollahi2016b}. In \citet{Abdollahi2016b}, the latter approach was optimized by introducing a Boltzmann machine to simultaneously optimize the recommendation and explanations. 
%Providing interpretability through similarity of user behavior is shallow. It does not allow a user to judge if the model learns the right thing. 
%However, \citet{Bellini2018} go with their work in a similar direction. They train a knowledge-aware autoencoder for explainable recommendations with categories and properties from DBpedia \citep{Auer2007}. The movie recommendation by its popularity among similar users and by the personalization of the model \citep{Bellini2018}. That means, they show the user that the model recommends a movie because the user liked a similar movie and prefers the recommended movie over another movie. However, this still does not allow the user to understand the model's behavior fully. Thus, full interpretability is not given. 
%\citet{Xiao2017} go one step further and explain the model's behavior. They do so by introducing an attentional factorization machine (FM) to the recommender task. Their method learns a neural attention network that reflects the importance of each feature interaction in \ac{fm}. The attention values can be used as explanations of the models' behavior \citep{Xiao2017}. However, the neural attention network itself is a black box. Thus, their model is only partially interpretable. 
\citet{Xie2017} proposes \emph{ITransF}. \emph{ITransF} also relies on the attention concept to create an interpretable model. \emph{ITransF} consists of a translational embedding method similar to \emph{STransE} \citep{Nguyen2016}. In addition, they learn sparse attention vectors. The sparse attention vectors reflect how important a concept dimension is for the classification, and thus help to understand how different relations share concepts \citep{Xie2017}. 
\emph{TEM} is another method relying on the attention approach to establish interpretability \citep{Wang2018}. First,\emph{TEM} uses a Decision tree to learn decision rules. Next, they design an attention network-based embedding model that uses those decision rules as features. The attention network guarantees that the recommendation process is fully interpretable \citep{Wang2018}.
Attention approaches are not the only way the literature explores to introduce interpretability in sub-symbolic approaches. \citet{anelliHowMakeLatent2019} introduces an interpretable recommender system relying on an \ac{fm}. The latent factors of the \ac{fm} are initialized by semantic features coming from a knowledge graph \citep{anelliHowMakeLatent2019}. In addition, semantic features are injected into the learning process. \citet{anelliHowMakeLatent2019} show that their approach allows conserving the informativeness of the entities in the knowledge graph in the learned recommender model. \citet{anelliHowMakeLatent2019} claim that this guarantees the interpretability of the models' recommendations. 
\emph{CrossE} \citep{Zhang2019a} is a sub-symbolic embedding for link prediction that explains by analogy. \emph{CrossE} predicts missing links by a translational model. Post-hoc, \emph{CrossE} generates explanations of the predicted link. It does so by finding closed paths from the head to the predicted tail entity. Next, it searches for similar structured paths in the knowledge graph between entities already connected by the predicted relationship \citep{Zhang2019a}. The found paths are shown to the user to justify the models' predicted link \citep{Zhang2019a}. 
Another embedding-based approach is called \emph{INK} \citep{Steenwinckel2022}. \emph{INK} is used to create embeddings of nodes given their neighborhood. The embeddings may be used in further \ac{ml} models for node-level classification \citep{Steenwinckel2022}. \emph{INK} makes a symbolic binary feature representation of the node's neighborhood for every embedded node. The binary features allow humans to interpret and understand the embedding created by \emph{INK} \citep{Steenwinckel2022}. \citet{Steenwinckel2022} show that \emph{INK} performance is similar to the state-of-the-art black-box algorithms \emph{R-GCN} \citep{Schlichtkrull2018} and \emph{RDF2Vec} \citep{Ristoski2016}.

\emph{RuleRec} \citep{Ma2019} is a neuro-symbolic recommender system that starts from a rule-based approach. It first mines rules together with a probability of finding a path connecting items pairs with that rule. A standard matrix factorization algorithm is then used for the actual recommendations. The mined rules and corresponding probabilities augment the matrix factorization algorithm \citep{Ma2019}. \citet{Ma2019} show that this leads to a better generalization ability when dealing with cold-start issues of recommender systems. 
Another method combining rule-based learning and embedding methods is proposed by \citet{Ai_2018}. The authors use at the core of their approach a translation function similar to \emph{TransE} \citep{Bordes2013}. The translational function of \emph{TransE} is extended to reflect the probability of a tail entity given a head entity and a corresponding relation. Gradient descent is deployed to optimize the probability for all triples in the training set. The embedding is then used to predict missing links \citep{Ai_2018}. After a missing link is predicted, the model generates an explanation \citep{Ai_2018}. First, possible closed paths between the head and tail entity are generated by breadth-first search. Next, the probability for each path is calculated by the translational function. The path with the highest probability is shown to a user to explain the predicted link \citep{Ai_2018}
\citet{Ruschel2019} propose a similar approach. However, they focus on the link prediction task instead of the recommendation task and use \emph{SFE} \citep{Gardner2015, Gusmao2018}, a performance version of \emph{PRA} \citep{Lao2011}, to mine rules used as explanations. 
\citet{Polleti2020} also combine a rule mining and embedding method to compute interpretable recommendations. However, they add counterfactuals to their explanation. Thus, they do not simply justify why the user should trust the recommendation, but also why it should not trust it. They do so by implementing Snedegar's theory of reasoning. For example, they select reasons, i.e., paths through the knowledge graph, against a recommendation by searching for reasons in favor of a competing recommendation that the initial recommendation is not satisfying \citep{Polleti2020}. 

%\subsection{Neuro-Symbolic Approaches to Interpretable Machine Learning on Knowledge Graphs}
%The latter research directions to machine learning with knowledge graphs focus mainly on a symbolic or sub-symbolic representation of the knowledge graph. However, methods relying on symbolic representation suffer from scalability issues while being highly interpretable. And methods relying on sub-symbolic representation are highly scalable, but interpretability is hard to achieve. 
%The following approaches use both types of representation to establish scalable and explainable machine learning methods on knowledge graphs. 
%\emph{RuLES} \citep{Ho2018}, for example, learns rules guided by a knowledge graph embedding. At each iteration, \emph{RuLES} expands existing rules such that the link prediction performance is optimized. The knowledge graph embedding provides the probability of a rule to be expanded by an atom \citep{Ho2018}. That way, the search space for new rules is pruned, which increases the scalability \emph{RuLES} compared to other rule-mining methods. 
%Another method combining rule-based learning and embedding methods is proposed by \citet{Ai_2018}. The authors use at the core of their approach a translation function similar to \emph{TransE} \citep{Bordes2013}. The translational function of \emph{TransE} is extended to reflect the probability of a tail entity given a head entity and a corresponding relation. Gradient descent is deployed to optimize the probability for all triples in the training set. The embedding is then used to predict missing links \citep{Ai_2018}. After a missing link is predicted, the model generates an explanation \citep{Ai_2018}. First, possible closed paths between the head and tail entity are generated by breadth-first search. Next, the probability for each path is calculated by the translational function. The path with the highest probability is shown to a user to explain the predicted link \citep{Ai_2018}
%\citet{Ruschel2019} propose a similar approach. However, they focus on the link prediction task instead of the recommendation task and use \emph{SFE} \citep{Gardner2015, Gusmao2018}, a performance version of \emph{PRA} \citep{Lao2011}, to mine rules used as explanations. 
%\citet{Polleti2020} also combine a rule mining and embedding method to compute interpretable recommendations. However, they add counterfactuals to their explanation. Thus, they do not simply justify why the user should trust the recommendation, but also why it should not trust it. They do so by implementing Snedegar's theory of reasoning. For example, they select reasons, i.e., paths through the knowledge graph, against a recommendation by searching for reasons in favor of a competing recommendation that the initial recommendation is not satisfying \citep{Polleti2020}. 
%\emph{RuleRec} \citep{Ma2019} is a neuro-symbolic recommender system that starts from a rule-based approach. It first mines rules together with a probability of finding a path connecting items pairs with that rule. A standard matrix factorization algorithm is then used for the actual recommendations. The mined rules and corresponding probabilities augment the matrix factorization algorithm \citep{Ma2019}. \citet{Ma2019} show that this leads to a better generalization ability when dealing with cold-start issues of recommender systems. 

%\subsection{Other Approaches to Interpretable Machine Learning on Knowledge Graphs}

The comprehensibility of \acp{kg} is even leveraged to interpret neuro-symbolic approaches for image classification \citep{Alirezaie2018}.
\citet{Alirezaie2018} trained a convolutional autoencoder (CAE) to segment and classify satellite images. A second CAE reconstructs the initial image from the output of the first CEA \citep{Alirezaie2018}. The authors argue that segmenting and classifying CAE is prone to misclassification in regions where the reconstruction is faulty. They extract the features from those regions and use them to apply geospatial reasoning with the OntoCity knowledge graph \citep{Alirezaie2018}. The reasoning identifies the most related concept from the misclassification and the region type \citep{Alirezaie2018}. This, for example, allows recognizing errors like classifying a shadow as water by reasoning that a building is next to that segment and shadows create a similar color to the water in the satellite pictures. Finally, \citet{Alirezaie2018} communicates the explanations for the misclassification to the user. 

\begin{table}[!ht]
\centering
\footnotesize
    \begin{tabular}{p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm}}
    \toprule
    \rotatebox{60}{Reference}           & \rotatebox{60}{Representation}    & \rotatebox{60}{Setting} &  \rotatebox{60}{Task}  & \rotatebox{60}{Learning}  & \rotatebox{60}{Comprehensibility} \\
    \toprule
    \citep{Lao2011}                & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\ 
    \citep{Barati2016}                & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\ 
    \citep{Omran2018}               & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\ 
    \citep{Wang2015}               & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\ 
    \citep{Galarraga2015}               & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\ 
    \citep{Chen2016a}               & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\ 
    \citep{Meilicke2019}               & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\
    \citep{Ott2020}                 & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\
    \citep{Yang2017}               & \emph{NSB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\
    \citep{Sadeghian2019}           & \emph{NSB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\
    \citep{Das2017}  & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rl}     & \ac{iml} \\
    \citep{Lin2018}  & \emph{SB}    & \emph{KAQ}       & \ac{lp} & \ac{rl}     & \ac{iml} \\
    \citep{Bhowmik2020}  & \emph{SB}    & \emph{KAQ}      & \ac{lp} & \ac{rl}     & \ac{iml} \\
    \citep{Xian2019} & \emph{SB}    & \emph{KAW}      & \ac{r} & \ac{rl}     & \ac{iml} \\
    \citep{Zhang2020} & \emph{SB}    & \emph{KAW}      & \ac{r} & \ac{rl}     & \ac{iml} \\
    \citep{Zhu2021} & \emph{SB}    & \emph{KAW}      & \ac{r} & \ac{rl}     & \ac{iml} \\
    \citep{Zhu2021} & \emph{SB}    & \emph{KAW}      & \ac{r} & \ac{rl}     & \ac{iml} \\
    \citep{Abdollahi2016a}                 & \emph{SSB}    & \emph{KAW}       & \ac{r} & \ac{fm}     & \ac{iml} \\ 
    \citep{Xiao2017}                 & \emph{SSB}    & \emph{KAW}       & \ac{r} & \ac{fm}     & \ac{iml} \\ 
    \citep{Xie2017} & \emph{SSB}    & \emph{KAQ}                & \ac{lp} & T     & \ac{iml} \\ 
    \citep{Wang2018} & \emph{SSB}    & \emph{KAW}                & \ac{r} & TB    & \ac{iml} \\ 
    \citep{anelliHowMakeLatent2019} & \emph{SSB}    & \emph{KAW}               & \ac{r} & \ac{fm}    & \ac{iml} \\
    \citep{Zhang2019a}  & \emph{SSB}    & \emph{KAQ} & \ac{lp}               & T    & \ac{iml} \\ 
    \citep{Steenwinckel2022} & \emph{SSB}    & \emph{KAQ}                & \ac{nc} & \ac{ann}    & \ac{iml} \\
    \citep{Ho2018}                 & \emph{NSB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\
    \citep{Ai_2018}                 & \emph{NSB}    & \emph{KAW}       & \ac{r} & \ac{kge}     & \ac{iml} \\ 
    \citep{Ruschel2019}                 & \emph{NSB}    & \emph{KAQ}       & \ac{lp} & \ac{rbl}     & \ac{iml} \\
    \citep{Polleti2020}                 & \emph{NSB}    & \emph{KAW}       & \ac{r} & \ac{kge}     & \ac{iml} \\ 
    \citep{Ma2019}                 & \emph{NSB}    & \emph{KAW}       & \ac{r} & \ac{rbl}     & \ac{iml} \\ 
    \citep{Alirezaie2018}               & \emph{NSB}    & \emph{KAW}       & Other & \ac{ann}     & \ac{iml} \\ 
    \end{tabular}
    \normalsize
\caption{Literature review table of \acs{kg}s for \ac{iml}}\label{tab:scop}
\end{table}

%TODO: Überleitung
%-------------------------------------------
\subsection{\acs{kg}s for \ac{xai}}\label{sub:kgforxai}
%-------Simon locked, 15.04.22-------
Publications dealing with \acp{kg} in order to augment the explainability of \ac{ml} models surged recently \citet{Hitzler2020NeuralsymbolicIA, Lcu2019OnTR}. Recalling that \ac{xai} is the mapping of the output of a \ac{ml} model to its corresponding input (see subsection~\ref{sub:comp}), those approaches that use \acp{kg} for \ac{xai} shall be regarded in the following.

%-------------------------------------------
\subsubsection*{\ac{rbl} applications of \acs{kg}s for \ac{xai}}
As mentioned in subsection~\ref{sub_hist}, abstract forms of \acp{kg} were used in order to generate knowledge or define rules already in the end of the $20^{th}$ century.
%-------------------------------------------
A vivid example is given by \citet{Towell1991}, who introduced \acfp{knn}, in order to refine symbolic knowledge. Essentially, the authors approximated an knowledge network (DNA sequences) by learning from a set of rules that are assumed to stem from this network. 
%-------------------------------------------
Furthermore, \citet{Fayyad1996FromDM} described the potential application of probabilistic graphic dependency models for the classification of bank customers based on loan and income characterizations.
%-------------------------------------------
The notion of graphs and especially \acp{kg} came hand in glove with the raise linked datasets. \citet{Huang2009} for instance, used graph analysis to detect patterns within textual documents from domains such as terrorist or biological networks, while other authors like \citet{dAquin2012CombiningDM} focused more on the automation of knowledge acquisition from multiple data sources in order to conduct inference and reasoning. In fact, \citet{dAquin2013InterpretingDM} even deepened their efforts by sequential pattern extraction, a dedicated data mining method based on linked data in order to produce explainable insights into students' course enrolment datasets.
%-------------------------------------------
With the surge of the semantic web thus, concepts from publicly available linked datasets were incorporated in \ac{kg} databases such as \emph{DBpedia}. Amongst others, \citet{Paulheim2012} introduced an application for graph-based hypothesis generation to explain statistics called \emph{Explain-a-LOD}, which is based on \emph{Linked Open Data}. Thus, as a direct successor, \emph{ViCoMap}, added map-based visualizations and allowed for an even more explainable interpretation of statistical data \citep{Ristoski2015}. Thereby, a RDF dataset, is being explored automatically via RapidMiner by the LOD extension. Figure~\ref{fig:vcm} displays the simplified framework of \emph{ViCoMap}.

\begin{figure}[!ht]
  \centering
  %TODO: Grafik evtl entfernen.
  \includegraphics[scale=0.45]{figures/akt_ViCoMap.png}
  \caption{Simplified framework of \emph{ViCoMap}, taken from \citep{Ristoski2015}.}\label{fig:vcm}
\end{figure}

%-------------------------------------------
\subsubsection*{\acs{gnn}-based applications of \acs{kg}s for \ac{xai}}
Formally, the prediction of a \ac{gnn} $\hat{y}$ is given by $\hat{y} = \phi(G_w(v), X_w(v))$, whereby $G_w(v)$ is the \ac{kg} information and $X_w(v)$ is the vertex information.
%-------------------------------------------
Firstly, \citet{NEURIPS2019_d80b7040} provided an approach to explain predictions of a \ac{gnn}, named \emph{GNNExplainer}. The system highlights those modules of the \ac{gnn}, that determine the prediction in particular by learning those potential explanations. The technique is based on the assumption that the gradient of the prediction is known and the underlying data is \acf{iid}. Hence, it generates an explanation for $\hat{y}$ as $(G_S, X_S^F)$, where $G_S$ is a subgraph of the computation graph and $X_S^F$ are those vertex features being most important for $\hat{y}$. Thereby, a vital component of \emph{GNNExplainer} is learning real-valued \emph{graph- and feature-masks} $M$.
%-------------------------------------------
A major drawback of the previously mentioned \ac{gnn} prediction explanations are based on the assumption that the gradient of the model is known so that explanations can be learned. Those techniques are thus not model-agnostic and in those cases where only the output of a black-box model is given, they are not applicable. More recently, \citet{Zhang2021} addresses the underlying \ac{iid} assumption of for instance \emph{GNNExplainer}. The authors introduce \emph{RelEx}, which is a model-agnostic \ac{gnn} explainer, being able to achieve comparable or better performance than \ac{iid} explanation models. 
%------------------------------------------
Another representative from the field of model-agnostic \ac{gnn} explainers is \citet{Vu2020}. Referred to as \emph{\acf{pgm} explainer}, the authors' manage to identify pivotal graph
components and to deduce explanations in the form of a graphical model and conditional probabilities. Thereby, \acp{pgm} use graph-based representation to encode complex distributions over a multi-dimensional space. Compared to \emph{GNNExplainer}. Figure~\ref{fig:pgm} displays the exemplary \ac{pgm} explainer framework compared to \emph{GNNExplainer}, \emph{\acf{pgm} explainer} would provide an explanation in the form of Bayesian network that estimates the probability of a node $E$ has the predicted role given a realization of other nodes. %It is thus less prone to 

\begin{figure}[!ht]
  \centering
  %TODO: Grafik evtl neu malen.
  \includegraphics[scale=0.3]{figures/akt_pgm.png}
  \caption{Exemplary \ac{pgm} explainer framework compared to \emph{GNNExplainer}, taken from \citep{Vu2020}.}\label{fig:pgm}
\end{figure}

\emph{\acf{pgm} explainer} is, as well, model-agnostic and thus, especially when it comes to practical application, does not rely on an explained model, which epitomizes a crucial advantage. Furthermore, the model is applicable to other graphical models such as Dependency networks or Markov networks.

% \citet{Luo2020} PGExplainer; trains an deep nn to parameterize the generation process of explanations to provide global explanations of any gnn
%\citet{Gad-Elrad2020} for any embedding method -> make cluster -> label clusters by rules from kg 

%------------------------------------------- Local
Besides constructing relevant walks, one can also shad some light on the proximity of a vertex of a \ac{kg}, whose prediction is to be explained. In 2020, \citet{Huang2020} proposed \emph{GraphLIME} to explain any vertex $v_i$ by a set of features $\zeta(v)$. Features are assumed to be extracted from the real world, can be understood by humans and are associated to a vertex via a so-called feature vector $x_i$. Next, the authors define a set of neighbours $S_N$ of a vertex $v$, also referred to as the network of $v$, by the nodes whose distance from $v$ is within $N$ hops and links. Eventually, the nonlinear, feature-wise kernelized \emph{Hilbert-Schmidt Independence Criterion (HSIC) Lasso}  method is used to determine the $K$ least redundant feature vectors. This method is a vast supervised feature selection method and can be revised in \citet{Yamada2016}. Essentially, the framework proposed by the authors learns a non-linear interpretable model (the HSIC Lasso explanation model) in the local proximity of a predicted vertex. This surrogate model is referred to as non-linear, because it takes the graph structure information into account and can thus be seen as opposed to \emph{LIME}, a linear explanation model \citep{Ribeiro2016}. Experimenting with the real-world datasets \emph{CORA} and \emph{Pubmed}, the explanations of \emph{GraphLIME} are depicted as more descriptive, when compared to \emph{LIME} or \emph{GNNExplainer}.

\begin{figure}[!ht]
    \begin{minipage}[b]{0.63\linewidth}
      \centering
      \includegraphics[scale=0.8]{figures/akt_graphlime.png}
      \caption{Generic components of \emph{GraphLIME}.}\label{fig:glm}
    \end{minipage}
    \begin{minipage}[b]{0.335\linewidth}
        Figure~\ref{fig:glm} displays the generic components of \emph{GraphLIME}, with vertex $v_1$, whose prediction is to be explained, vertices $v_2$, $v_3$ and $v_4$, which are in the proximity of $v_1$ and whereof the feature vectors of $v_2$ and $v_3$ form $\zeta(v)$. Here, $N=1$, which is why $v_5$ is not within $S_N$.
    \end{minipage}
\end{figure}

%------------------------------------------- Local
Another representative of the group of local \ac{gnn} explanation methods was introduced by \citet{Duval2021} in 2021. Again, \emph{GraphSVX} is based on a surrogate model to explain a predicted vertex locally. On the node-level, the proposed method computes the marginal contribution $f(X', A')$ of nodes and features using the surrogate model binary masks $(M_N, M_F)$. Eventually, \emph{GraphSVX} draws on the so-called \emph{Shapely value}, a concept from game theory, which represents the fair distribution of gains in a game. The authors approximate this metric in order to create a real signification of an explanation obtained by \emph{GraphSVX}. Additionally, the authors describe a unified framework of \ac{gnn} explanations, consisting of a \emph{mask generator}, a \emph{graph generator} and an \emph{explanation generator}, in which they locate competing models, such as \emph{GNNExplainer}, \emph{PGExplainer}, \emph{PGM-Explainer} or \emph{GraphLIME}.

Even though \citet{Duval2021} use a super-ordinate graph for generating explanations, the scope of \emph{GraphSVX} is limited to node level predictions. \emph{GraphSHAP}, introduced by \citet{Perotti2022} in 2022 jointly makes use of the \emph{Shapely value}, but on a graph classification level. Since the scope of this survey is limited, further details shall be spared out. However, table~\ref{tab:mask} shall convey a brief comparison of the above-described, mask-based approaches to \ac{gnn} explanation.

% TODO: Plot the unified framework.

\begin{table}[!ht]
\centering
\footnotesize
    \begin{tabular}{ttttt}
    \toprule
    {Model}         & {Masking} & {Loss}    & {Surrogate model}  & {Explanation} \\
    \toprule
    GNNExplainer    & Yes       &  $MI(Y, (M_E, M_F))$   & No    & Masks \\ 
    \bottomrule
    \end{tabular}
    \normalsize
\caption{Comparison of mask-based \ac{gnn} explainers}\label{tab:mask}
\end{table}

%------------------------------------------- Global
One of the most popular approaches to incorporating \ac{xai} to \acp{gnn} was delivered by \citet{Schnake2020}, who elaborated on high-order explanations of \acp{gnn} via so-called relevant walks. The authors managed to identify groups of edges that commonly contribute to the \ac{gnn} prediction by using a nested attribution scheme. At each step of this scheme, \acf{lrp}, a technique introduced by one of the authors earlier (see \citet{Bach2015, Montavon2019}, can be applied in order to determine relevance. In accordance with our definition of \ac{xai}, the \ac{gnn} \ac{lrp} method explains any \ac{gnn} prediction by extracting the most relevant \emph{paths} from the input to the output of the \ac{gnn}. Here, paths correspond to \emph{walks} on the input graph $G$. The method is based on \emph{high-order} Taylor expansions of the \ac{gnn} output as well as chain-rules that are used to extracting the Taylor expansion's terms \citep{Bach2015}. Eventually, the \ac{gnn} \ac{lrp} method is transferable to large, nonlinear models. The method is applicable to a vast range of \acp{gnn} architectures and is set for application in sentiment analysis of text data, structure-property relationships in quantum chemistry, and image classification \citep{Montavon2019}. A detailed description of the \ac{gnn} \ac{lrp} method would exceed the scope of this survey, which is why figure~\ref{fig:lrp} shall summarize the proceeding and the \citet{Schnake2020} shall be recommended for in-depth explanations.

\begin{figure}[!ht]
  \centering
  %TODO: Grafik evtl neu malen.
  \includegraphics[scale=0.3]{figures/akt_gnn_lrp.png}
  \caption{Exemplary \ac{pgm} \ac{lrp} method, taken from \citep{Montavon2019}.}\label{fig:lrp}
\end{figure}

%------------------------------------------- Symbolic, Global and local, model-agnostic
Yet another model-agnostic but symbolic post-hoc explanation method for graph classifiers was proposed by \citet{Abrate2021} in 2021. The above-mentioned creation of counterfactuals comes into play, being used to construct a so-called \emph{counterfactual graph}. The method proposed by the authors is a heuristic search schema that can be conducted in two variants: \emph{Oblivious} (the algorithm searches for the optimal counterfactual graph by querying the black-box graph classifier and abstracting the original graph) or \emph{data-driven} (the algorithm gains additional access to a subset, superset or the original training dataset of the black-box classifier). Similar to \emph{SHAP} \citet{Lundberg2017} and \emph{LIME} \citet{Ribeiro2016}, the authors thus rank statistics about the input data in order to achieve explainability - however by creating many counterfactual graphs for a given graph and stressing the most frequent edges eventually. Being apt for aggregation (creating counterfactual graphs for different input data), the approach of \citet{Abrate2021} can thus be described as global and model-agnostic. The authors forgo on integrating higher-order structures or graph properties into their approach.

%------------------------------------------- 
A major issue for \ac{xai} in \ac{kg}-based models is the occurrence of cyclic relations in the \ac{kg}. Cycles occur when edges relate vertices in contradictory hierarchies, as figure~\ref{fig:cyc} displays.

\begin{figure}[!ht]
    \begin{minipage}[b]{0.63\linewidth}
      \centering
      \includegraphics[scale=0.5]{figures/akt_KG_cycles.png}
      \caption{Schematic example of \ac{kg} cycles.}\label{fig:cyc}
    \end{minipage}
    \begin{minipage}[b]{0.335\linewidth}
        The main issue if a \ac{kg} cycle is that reasoning over the graph in the form of choosing parent concepts within the \ac{kg} hierarchy for generating explanations is rendered nondeterministic \citep{Sarker2020}. Here, the edge $home-of$ would have to be broken in order to allow for deterministic reasoning. 
    \end{minipage}
\end{figure}

\citet{Sarker2020} address this issue by providing a circle-free version of the existing \emph{Wikipedia} \ac{kg}. Using \emph{breadth-first search (BFS)}, the authors break cyclic relations within the \ac{kg} and thus create the so-called \emph{Wikipedia} \ac{kg} \emph{(WKG)}. Interestingly, the authors introduce a measure for the \ac{xai}-related quality of their \ac{kg}, using a \ac{ilp}-based metric focusing on string similarity, which shall not be detailed here but can be revised in the original paper (\citep{Sarker2020}) in conjunction with \citet{Levenshtein75}. For final evaluation, a public available image classification dataset is, with annotations, cased into an \ac{owl} ontology and explanations are tried to be extracted using \emph{(WKG)} and existing \acp{kg} that still have cyclic relations such as \emph{DBpedia}. Eventually, the authors stipulate higher efficiency whilst minimal information loss by breaking cyclic relations.

%------------------------------------------- 
% \citet{Donadello2021} aligns dnn output with kg and than applies reasoning as explanations.

%------------------------------------------- Symbolic, global
Beneath \emph{WKG}, other approaches based on the exploitation of semantic information exist. \citet{Dragoni2022} for instance, constructs a logical reasoning flow, referred to as \emph{explanation graph}. The graph fulfills the formal criteria of a \ac{kg}, as defined in section~\ref{sec:ov} but differs from previously described approaches since it maps concepts used by humans to numeric features of a black box model. In fact, the authors aim at rendering an explanation in logical language format. For that, they created a framework being able to process semantic information from a knowledge base, referred to as semantic features $A_i$, based on the work of \citep{Doran2018}. In brief, semantic features represent the common attributes of an object, such as $3-Series \hookleftarrow (Car, BMW)$ and essentially are one kind of predicates of a First-Order Logic (FOL) expression $P$. The other kind of predicate are the output symbols of a black-box model $O_i$ that are to be rendered comprehensible. Hence, being graph-based, the authors define their system as consisting of unary predicates $O_i, A_i$ as vertices and the logic relations between those predicates, coming from an \ac{ai} system, as edges. The explanation graph hence combines singular knowledge fragments into a semantic reasoning system and thus creates explainability.

% TODO: Zeichnen.

%------------------------------------------- 
After having outlined the state of the art of \ac{kg} methods for \ac{xai}, table~\ref{tab:scop} displays the results of the literature review for this section.

\begin{table}[!ht]
\centering
\footnotesize
    \begin{tabular}{p{3cm} p{2cm} p{2cm} p{2cm} p{2cm}}
    \toprule
    \rotatebox{60}{Reference}           & \rotatebox{60}{Representation}    & \rotatebox{60}{Setting}  & \rotatebox{60}{Task}  & \rotatebox{60}{Learning}  \\
    \toprule
    \citep{Towell1991}                  & \emph{SSB}                        & \emph{KAQ}                & \emph{}             & \ac{rbl}      \\ 
    \citep{Fayyad1996FromDM}            & \emph{SSB}                        & \emph{KAQ}                & \emph{}             & \ac{rbl}      \\ 
    \citep{Huang2009}                   & \emph{SSB}                        & \emph{KAW}                & \emph{}             & \emph{RB}     \\    
    \citep{dAquin2012CombiningDM}       & \emph{SSB}                        & \emph{KAW}                & \emph{}             & \ac{rbl}     \\ 
    \citep{dAquin2013InterpretingDM}    & \emph{SSB}                        & \emph{KAQ}                & \emph{}             & \ac{gnn}      \\
    \citep{Paulheim2012}                & \emph{SSB}                        & \emph{KAW}                & \emph{}             & \ac{rbl}      \\
    \citep{Ristoski2015}                & \emph{SSB}                        & \emph{KAW}                & \emph{}             & \ac{rbl}      \\
    % Ristoski2015 includes visual interpretability.
    \citep{NEURIPS2019_d80b7040}        & \emph{SSB}                        & \emph{KAQ}                & \emph{}             & \ac{gnn}      \\
    \citep{Zhang2021}                   & \emph{SSB}                        & \emph{KAQ}                & \emph{}             & \ac{gnn} node level   \\
    \citep{Vu2020}                      & \emph{SSB}                        & \emph{KAQ}                & \emph{}             & \ac{gnn} node level  \\
    \citep{Schnake2020}                 & \emph{SSB}                        & \emph{KAW}                & \emph{}             & \ac{gnn} any level  \\
    \citep{Huang2020}                   & \emph{SSB}                        & \emph{KAW}                & \emph{}             & \ac{gnn} node level  \\
    \citep{Abrate2021}                  & \emph{SB}                         & \emph{KAW}                & \emph{GC}             & Other  & \ac{xai}\\
    \citep{Sarker2020}                  & \emph{SB}                         & \emph{KAW}                & \emph{GC}             & Other & \ac{xai}\\
    \citep{Dragoni2022}     & \emph{SB}                         & \emph{KAW}                & Other             & Other & \ac{xai}\\
    \bottomrule
    \end{tabular}
    \normalsize
\caption{Literature review table of \acs{kg}s for \ac{xai}}\label{tab:scop}
\end{table}

% Link-prediction \emph{LP}, Node-prediction \emph{NP}, Node-classification \emph{NC}, Graph-classification \emph{GC}, Clustering \emph{C}, Recommendation \emph{R}.  \\

The following section shall conclude the literature review and provide an outlook for future research in the field of \acp{kg} for \ac{cai}.


% \citep{Dervakos2022} explainable method. noch nicht peer-reviewed. Scheint es aber wert erwähnt zu werden.  

==> sections/knowledge_acquisition.tex <==
%-------------------------------------------
\section{\acs{kg}s for knowledge acquisition}
%-------------------------------------------

%-------------------------------------------
\subsection{\acs{kg} completion}

%-------------------------------------------
\subsection{\acs{kg} node classification}


==> sections/knowledge_aware_applications.tex <==
%-------------------------------------------
\section{\acs{kg}s for knowledge aware applications}
%-------------------------------------------

%-------------------------------------------
\subsection{\acs{kg} clustering}

%-------------------------------------------
\subsection{\acs{kg} recommender systems}


==> sections/methodology_and_definitions.tex <==
%-------------------------------------------
\section{Methodology and Definitions}\label{sub:meth}
%-------------------------------------------

%-------------------------------------------
\subsection{\acs{kg}s}\label{sub:kg}

A \ac{kg} is a directed labelled graph \citep{Hogan2021}. % definition 
Figure \ref{fig:running_example_kg} depicts a \ac{kg}.

\begin{figure}[!ht]
  \centering
  \includegraphics[scale=0.35]{figures/running_kg_example.png}
  \caption{Car manufacturer knowledge graph}\label{fig:running_example_kg}
\end{figure}

In general, a graph is a set of connected entities. 
Frequently, entities are referred to as \emph{vertices} $v$ (or \emph{nodes}), while connectors are referred to as \emph{edges} $e$ (or \emph{links}), in the context of a graph.
%\acp{kg}. 
Thus, a 
% \ac{kg} 
graph $U$ consists of a set of vertices $V = \{v_1, v_2, v_3, ..., v_i, ..., v_n\}$ and edges $E = \{e_1, e_2, e_3, ..., e_j, ..., e_m\}$. % for any $v_i \in N$ and $e_j \in M$ with $1 \leq i < n$ and $1 \leq j < m$.  <- not necessary and wrong because (n not in N) and (m not in M) and what is N/M?
This renders a 
%\ac{kg} 
graph $U$ as a subset of $V \times E \times V$ \citep{sanchez-lengelingGentleIntroductionGraph2021}.

A directed graph is a graph in which edges have a direction. Thus, given a directed edge $e_1$ from vertex $v_1$ to vertex $v_2$, graph traversal via $e_1$ is exclusively possible from $v_1$ to $v_2$ and not vice versa \citep{Harary1965}.

A labelled graph is a graph in whifh holds $ \forall v_i \in V$ and $ \forall e_j \in E$ that exactly one element from a set of symbols $S = \{s_1, s_2, s_3, ..., s_k, ..., s_o\}$ is assigned to them. A symbol $s_k$ is, in general, the name of an entity like "\emph{Ute}" or "\emph{Munich}" or the name of a relationship like "\emph{is-model-of}"\citep{Gallian2001}.

Due to the latter properties, a \ac{kg} is optimal for storing highly relational data while preserving its semantics and allowing for deductive reasoning. 

The following paragraphs shall outline \ac{kg} representations in description logic and as a matrix. Those paragraphs shall set the ground for exploring knowledge-aware systems, knowledge acquisition, and \ac{cai} relying on \acp{kg} as an input. 

% In order to outline the basic terminology of the following sections, the following paragraphs shall outline two basic ways of representing \acp{kg}, firstly as an actual graph and secondly in an alternative way as a matrix. Subsequently, this subsection shall introduce the pivotal notion \acs{kge} and shall eventually outline how \acp{kg} are frequently applied in the context of \acs{ml}.

% fundament des KGs in der ALC

% \subsubsection*{\acs{kg}s in description logic}
\subsubsection*{Symbolic representation of \acs{kg}s}
\acs{kg}s are a form of knowledge bases and typically build a domain-specific ontology \citep{Hogan2021}. 

Let us consider the vertices and edges of a \acs{kg} from a knowledge base perspective. 
The vertices of a \acs{kg} can typically be divided into a schema and individuals \citep{Hogan2021}. 
The schema holds vertices that describe general concepts (i.e. the classes of individuals) like \emph{Plant}, or \emph{Car}, and relations between them. In addition, one might define general rules over concepts and relations, like in Equation \ref{eqn:works-in}, saying that \emph{A} \emph{works-in} \emph{C} if \emph{A} \emph{builds} \emph{B} and \emph{B} \emph{is-produced-in} \emph{C}.

\begin{equation}
works\mbox{-}in(A,C) \equiv builds(A,B) \sqcup is\mbox{-}produced\mbox{-}in(B,C)
\label{eqn:works-in}
\end{equation}

In contrast, individuals are concrete instances of the concepts, like a vertex \emph{Spartanburg} which is a member of the concept \emph{Plant}.
Furthermore, the semantics of the edge's symbols in a \acs{kg} typically imply rules. For example, the edge \emph{is-produced-in} has to be directed from an individual of the concept \emph{Car} to an individual of the concept \emph{Plant}. Therefore, an edge with the label \emph{is-produced-in} from and to individuals of any other concept would be semantically inconsistent.     

Ideas like concepts, individuals, and rules are hard to model in a purely graph-based representation. Description logic can help out with this problem \citep{Horrocks2008}. It allows representing the \acs{kg} in the form of a knowledge base. 
Descriptions logic defines a formal model of concepts, roles, individuals, and relations \citep{Baader2009}. 
$ALC$ is one variation of description logic \citep{Baader2009}. It describes the \acs{kg} as a knowledge base $K$ as an ordered set of a Terminological box ($TBox$)  and Assertional box ($ABox$) \citep{Baader2009}. A knowledge base in a description logical representation is formally defined in Equation \ref{def:kg_in_alc}.

\begin{equation}
    K=(TBox, ABox)
\label{def:kg_in_alc}
\end{equation}

The $TBox$ contains the schema of the knowledge base. The schema describes concepts and potential relations between those. 
Furthermore, rules that hold for a given concept and or relation can be defined in the $TBox$. 
The $ABox$ contains the ground truth as triples, i.e. individuals and their relations to concepts and other individuals, like \emph{Ute builds-a 3 Series} and \emph{X4 is-produced-in Spartanburg}. Please consult \citet{Baader2009} for a formal definition of the $TBox$ and $ABox$.

Representing a \acs{kg} as a knowledge base allows \ac{ai} applications to reason deductively within the domain of the \acs{kg} \citep{Grau2008}.


% hier noch eine überleitung
%-------------------------------------------
% make this to subsymbolic representation space of KGs
\subsubsection*{Sub-symbolic representation of \acs{kg}s}
% ---Christoph locked---
Besides representing a \acs{kg} as a graph or in symbolic description logic, the sub-symbolic representation of \acs{kg}s gained vast popularity with the rise of neural machine learning. 

The primary rationale of sub-symbolic KG representations is to map the knowledge graph with its nodes and edges in a low-dimensional numeric space. Common numeric spaces for embedding a KG are vector, matrix, or tensor spaces. However, the literature on knowledge graph embeddings continuously presents new and highly expressive representations. Moreover, the concrete expression levels of the embedding dimensions are often too complex to be set by a human-made mapping. Thus, the mapping is learned. 

Standard vector, matrix, and tensor space representations are explored in the following paragraphs. These are followed by examples of other expressive numeric spaces like the complex vector space, Gaussian space and manifolds.  

% evolution von #vector space (one hot encoding) 
\paragraph{Vector space representation}
The naive way of embedding a KG in vector space is by one-hot encodings. Each KG node and KG edge is embedded in a unique vector, with the total number of nodes and edges as its length. Each vector dimension is 0 or 1, and a vector sums up to 1. While this method is intuitive, it does not scale to larger KGs and becomes memory-wise prohibitively expensive.    
Various KG embedding methods that either compute, like node2vec \citep{Grover2016}, or learn \citep{Bordes2013} lower-dimensional vector space representation for each node and edge in a KG were proposed to overcome this limitation. 
%citep alot like node2vec HolIE ..
TransE \citep{Bordes2013} was in 2013 one of the first methods that learned a function to translate nodes and relations of a KG into $d$-dimensional vector space $\mathbb{R}^d$. An example of KG entities and relations represented by TransE embeddings is shown in Figure 1. 

% TODO: Figure schön machen
\noindent
\begin{minipage}%{0.4\textwidth}
\begin{tikzpicture}[scale=0.65]
\begin{axis}[
  axis line style={Stealth-Stealth},
  xmin=-4.,xmax=3.,ymin=-4.,ymax=3.,
  xtick distance=2,
  ytick distance=2,
  xlabel=$x$,
  ylabel=$y$,
  title={Representation of entities and relations in $\mathbb{R}^2$},
  grid=major,
  grid style={thin,densely dotted,black!20}]
\node[label={above:{3Series}},circle,fill,inner sep=1.5pt] at (axis cs:-2.,0.5) {};
\node[label={right:{BMW}},circle,fill,inner sep=1.5pt] at (axis cs:0,-3.5) {};
\node[label={right:{Ute}},circle,fill,inner sep=1.5pt] at (axis cs:-2.5,-3) {};
%vector at end
\coordinate (S) at (axis cs:0,0);
\coordinate (A) at (axis cs:0.5, 2.5);
\coordinate (B) at (axis cs:2.5, -2.5);
\coordinate (C) at (axis cs:2.5, -0.5);
%\draw[,very thick,->](S)--(A) node [midway, fill=white] {builds};
%\draw[,very thick,->](S)--(B) node [midway, fill=white] {model-of};
\draw[,very thick,->](S)--(C) node [midway, fill=white] {works-at};
\end{axis}
\end{tikzpicture}
\end{minipage}
\begin{minipage}%{.5\textwidth}
\begin{equation*} 
\begin{split}
    Ute = (-2.5, -3) \\
    BMW = (0, -3.5) \\
    3Series= (-2, 0.5) \\
    \vec{builds} = (0.5, 2.5) \\
    \vec{model\mbox{-}of} = (2.5, -2.5) \\
    \vec{works\mbox{-}at} = (2.5, -0.5)
\end{split}
\end{equation*}
\end{minipage}

Embedding a knowledge graph in the real-valued vector space limits the expressiveness of the embedding. Vector space embeddings struggle, for example, to embed n-to-n relationships \citep{Bordes2013}.
TransR \citep{Lin2015} overcomes this limitation by embedding entities in one vector space $\mathbb{R}^d$ and relationships in another vector space $\mathbb{R}^k$. A projection matrix $M_r \in \mathbb{R}^{k \times d}$ maps the entities in the vector space of the relationships \citep{Lin2015}. 

However, certain relationship properties like transitivity \citep{Schmidt2010} cannot be expressed by embedding a knowledge graph in the real-valued vector space \citep{Lin2015}. Thus, other sub-symbolic representation types of knowledge graphs like matrix representations were introduced.  

\paragraph{Matrix and Tensor Space Representation}
One natural approach to realize a sub-symbolic representation of the knowledge graph as a matrix is an adjacency matrix. 
The adjacency matrix of graph $U = \langle V,E \rangle$ is defined as the boolean $|V| \times |V|$ matrix that contains, at any coordinate $\langle v_i, v_j \rangle$, the value 1 if there is an edge connecting $ v_i$ and $v_j$ \citep{Biggs1993}.
However, the standard adjacency matrix does not express the label of the relationship. The adjacency matrix can be transformed into a 3-D tensor to add labeled relationship information. This tensor is defined as the boolean  $|V| \times |E| \times |V|$ tensor that contains, at any coordinate $\langle v_i, e_k, v_j \rangle$, the value 1 if the edge $e_k$ connects $v_i$ and $v_j$.
Those embedding methods become prohibitively expensive with a growing number of $|V|$ and $|E|$. 
RESCAL \citep{Nickel2011} mitigates this problem by applying tensor factorization to compute a compact tensor representation of $U$.
DistMult \citep{Yang2014} is an extension of RESCAL that decreases its computational expense further by restricting its relations matrices $W_r \in \mathbb{R}^{d\times d}$ to diagonal matrices. However, the restriction enforces that every relation is symmetric \citep{Schmidt2010}. This might lead to an unwanted representation of the KG \citep{Yang2014}.  
CP represents the knowledge graph as a canonical decomposition of tensors \citep{Hitchcock1927}. This is a tensor $X \in \mathbb{R}^{|V|, |E|, |V|}$ as a sum of $R$ rank one tensors $u_r^{v_i}\otimes u_r^{e_k}\otimes u_r^{v_j}$ where $r \in {1,..., R}$, $ u_r^e \in \mathbb{R}^{|E|}$, and $ u_r^v \in \mathbb{R}^{|V|}$ \citep{Lacroix2018}. Formally, tensor $X$ is defined as:

\begin{equation}
    X = \sum_{r=1}^{R} u_r^{v_i}\otimes u_r^{e_k}\otimes u_r^{v_j}
\end{equation}

Figure \ref{fig:cp} visualizes CP's representation of a KG triple $(v_i \   e_k \   v_j)$ in the tensor space. 

\begin{figure}[!ht]
  \centering
  \includegraphics[scale=0.5]{figures/cp_tensor.png}
  \caption{CP's representation of a KG triple $(v_i \   e_k \   v_j)$ in the tensor space \citep{Lacroix2018}. }\label{fig:cp}
\end{figure}


% TODO: Überleitung

% zu hochgradig spezifischen räumen wie: complex vector space, irrational, gaussian oder manifold
\paragraph{Complex Representation}
%rotatE
%Complex


%-------------------------------------------
%\subsubsection*{\acs{kge}s} % This should be a subsection like GNN "Kg representation in the complex vector space" 

%-------------------------------------------
\subsection{Representation learning}

%-------------------------------------------
\subsubsection*{\acs{kge}s}

%-------------------------------------------
\subsubsection*{Representation learning and \acs{gnn}s}\label{sub:gnn}
%-------Simon locked, 06.3.22-------READY FOR REVIEW
A \acs{gnn} is a transformation that can be optimized on all modules $V$ and $E$ of the graph, but also on the graph $U$ itself. Thereby, it preserves graph semantics and symmetry and is thus invariant to permutation \citep{scarselliGraphNeuralNetwork2009}. \acp{gnn} represent a special class of the conventional \acp{ann}, being capable of processing graph-structured data. In fact, the advent of conventional \acp{ann}, which can be traced back to \citet{McCulloch.1943}, \citet{ROSENBLATT.1958} and \citet{Minsky.1972}, resembles the current development of \acf{gnn} in a way that allows for the assumption that major applications of \acp{gnn} are yet to come. The prevalence of conventional \acp{ann} increased sharply when advances in computational hardware, such as the usage of \acp{gpu} for backpropagation, enabled \acp{ann} to approach human-like performance in diverse fields in the early 21st century \citep{Cire_an_2010}.\footnote{Since the scope of this survey is limited, conventional \acp{ann} cannot be outlined any further, but are detailed in \citet{Aggarwal.2018} and \citet{Goodfellow.2016}.} In the recent past, \acp{gnn} are increasingly being applied to major research fields, such as simulations in physics \citep{SanchezGonzalez2020LearningTS}, to antibacterial discoveries in biology \citep{Ackermann2020} and also to novel research areas like fake news detection \citep{Monti2019}. As outlined in subsection~\ref{sub:kg}, conventional graphs are to be distinguished from \acp{kg}. This subsection deals with \acp{gnn}, thus with a transformation that can be applied to both generic graphs and specific \acp{kg}. %In the following, the original \ac{gnn} model, proposed by \citet{scarselliGraphNeuralNetwork2009} in 2009 shall briefly be described. Subsequently, some relevant algorithms, such as \emph{DeepWalk} and \emph{GraphSage} shall be put into context.

%-------------------------------------------
%\paragraph*{The original \acs{gnn} model}
%First and foremost, Scarselli et al. distinguish applications to the graphical domain into two broad classes: graph-focused and node-focused applications.
\acp{gnn} process graphs as sets of units, whereby each unit has a certain \emph{state} $x_v$, beneath the above-mentioned modules $V$ and $E$ of a graph $U$. In the case of a \ac{kg}, labels $l$ can be processed by the \ac{gnn}. The state $x_v$ is determined by the so-called \emph{neighbourhood} $ne[v]$ of a vertex, which epitomizes all vertices connected to $v$ by an edge. Furthermore, $co[v]$ equates the set of edges with $V$ as a vertex. Within a \ac{gnn}, units update their states until a stable equilibrium is obtained. The equilibrium leads to the output $o_v$ of a \ac{gnn}. Hence, $o_v$ is computed for each node based on the state of the respective unit. \citet{scarselliGraphNeuralNetwork2009} summarizes state and output by so-called \emph{local transition (output) functions} as follows:

\begin{equation}\label{eq:gnn}
    \begin{aligned}[b]
        x_v & = f_w(l_v, l_{co[v]}, x_{ne[v]}, l_{ne[v]}) \\
        o_v & = g_w(x_n, l_v)
    \end{aligned}
\end{equation}

where $l_v$ is the label of the vertex, $l_{co[v]}$ is the label of the edges and $l_{ne[v]}$ the labels of the vertices in the neighbourhood of $v$. Note that especially $f_w$ can be displayed in compact form as $F_w(x,l)$ under the assumption that $x, l$ are the vectors obtained when summarizing all states and labels. $F_w(x,l)$ is referred to as \emph{global transition function} \citep{scarselliGraphNeuralNetwork2009, ZHOU202057}.

\newpage

\begin{figure}[!ht]
    \begin{minipage}[b]{0.53\linewidth}
    % TODO: Weitere Ebene mit Netzwerk hinzufügen.
      \centering
      \includegraphics[scale=0.35]{figures/akt_gnn.png}
      \caption{Generic construction of a \ac{gnn}.}\label{fig:gnn}
    \end{minipage}
    \begin{minipage}[b]{0.435\linewidth}
    For the construction of a \ac{gnn}, a method to solve \ref{eq:gnn}, a learning algorithm to optimize $f_w$ and $g_w$ and an implementation of $f_w$ is required. \citet{scarselliGraphNeuralNetwork2009} propose a computation of the state $x_v$ based on Banach's fixed point theorem in \citet{Khamsi2001}, leading to a so-called \emph{encoding network} analog to \acp{rnn} models \citep{Frasconi1998AGF}. Subsequently, a gradient-descent based learning algorithm that iteratively updates the states $x_n(t)$ until at time $T$ the original state is approximated by $x(T) \approx x$, computes the gradient and updates the weights $w$. Eventually, \citet{scarselliGraphNeuralNetwork2009} present an implementation of $f_w$ in a way that the global transition function $F_w$ equates a \emph{contraction map} w.r.t. $x$ as its \emph{fixed point}.
    \end{minipage}
\end{figure}

A contraction map is a function $F$ that maps one metric space into another under certain conditions \citep{Denardo1967}. Banach's fixed point theorem states that a contraction map $F_w$ on a complete metric space has a unique fixed point and that its iterative sequence converges to that fixed point (here: $x(T) \approx x$) \citep{Denardo1967, Khamsi2001}. Figure~\ref{fig:gnn} displays the generic construction of a \ac{gnn}, with the graph on the top, followed by its respective encoding network in the middle and the actual \ac{gnn}, obtained by unfolding the encoding network at the bottom. %\citet{scarselliGraphNeuralNetwork2009} implements $f_w$ and $g_w$ as feedforward \acp{ann}, while the encoding network is a \ac{rnn}.
In the unfolded \ac{gnn}, each layer refers to a point of time $t$ and contains all the units of the encoding network. This proceeding is referred to as constrained diffusion mechanism, already utilized in cellular neural networks \citep{Chua1988, Chua1988CellularNN, Kaluzny1992, Ogorzatek2005} and Hopfield neural networks \citep{Hopfield1982}.\footnote{The diffusion mechanism is constrained in order to assure the existence of a stable equilibrium. A more detailed discussion of the diffusion mechanism would exceed the scope of this survey but can be found in \citet{wang2021diffusion}.} In contrast to those however, \acp{gnn} do not require the specification of connectivity according to a predefined graph by using the above-displayed, more general diffusion mechanism \citep{scarselliGraphNeuralNetwork2009, ZHOU202057}. As figure~\ref{fig:gnn} unveils, connections between layers in an \ac{gnn} depend on the connectivity of the encoding network, not in a predefined graph.

%The relevant domain $D$ for \acp{gnn} is the cross-product of a set of graphs $U$ and a subset of their nodes $V$, thus $D = U \times V$.

%\begin{equation}
%    \begin{aligned}
%        L & = \{ ( U_i, v_{i,j}, t_{i,j}) \vert, U_i = (V_i, E_i) \in U; \\
%          & v_{i,j} \in V_i; t_{i,j} \in \mathbb{R}^m, 1 \le i \le p, 1	\le j \le q_i\}
%    \end{aligned}
%\end{equation}

%where $v_{i,j} \in V_i$ equates the $j$th vertex in a set $V_i \in V$ and $t_{i,j}$ denotes the desired association to $v_{i,j}$.

%In general, \citet{scarselliGraphNeuralNetwork2009} states that \acp{gnn} are a special case of \acp{rnn}, with some constraints, such as that the input graph is directed and acyclic. In the following, some special algorithms shall be outlined in order to set the stage for the further proceeding of this survey. 

%A comprehensive study on \acp{gnn} methods was provided by \citet{ZHOU202057}. \citet{ZHOU202057} also states three main limitations of this original \ac{gnn}:

%\begin{itemize}
%    \item The transition function $f$ is limited to be a contraction map, which is rather inefficient due to the iterative update of hidden states. 
%    \item The model is not suitable for learning a representation of relative positions of vertices instead of graphs, due to the unique required fixed point.
%\end{itemize}

It can be summarized that in general, \acp{gnn} are used to learn representations of vertices and edges of a \ac{kg}, which is called \emph{representation learning}. In the following sections, special types of \acp{gnn} will be put into context of knowledge aware systems, systems for knowledge acquisition as well as into the context of \ac{cai}.

% Aus meiner Sicht kein Platz für weitere Ausführungen an der Stelle...
%-------------------------------------------
%\paragraph*{DeepWalk}

%-------------------------------------------
%\paragraph*{GraphSage}

%-------------------------------------------
%\paragraph*{Spezifisch für KGs}

%-------------------------------------------
%\subsection{\acs{il}}
%-------Simon locked, 08.04.22-------
%\acf{il}, frequently referred to as inductive programming as well, can be understood as learning from logical but incomplete representations, such as learning of a dictionary from text \citep{Sakurai2001}. Recently, \acf{il} was applied to \acp{kg}, where, frequently, vertices or labels are incomplete, so that \ac{il} on \acp{kg} mostly relies on local connections for unknown vertices \citet{Wang2021, Hamaguchi2017}

%. (Hamaguchi et al. 2017) generates embeddingfor unseen nodes by aggregating the information from surrounding known nodes. (Teru, Denis, and Hamilton 2020) models relation prediction as a subgraph reasoning problem, and conducts inference solely based on the sampled subgraph structure. However, if unseen entities in CKGs have few links, structural-based methods cannot be applied directly. As an alternative, there exists work that incorporates entity description in the embedding process. This approach is inductive by nature. For example, (Xie et al. 2016) learns a joint embedding space for conventional entity embedding and description-based embedding using the CNN or the bagof-word (BOW) as an encoder, and (Li et al. 2016) distinguishes negative triplets from positive ones and incorporates LSTM as a textual encoder. Our work exploits both structure information and textual description for inductive learning on unseen entities

%-------------------------------------------
\subsection{State-of-the-art applications of \acs{kg}s}
%-------------------------------------------
%-------Simon locked, 14.04.22-------
The main purpose of this survey is to summarize the modern applications of \acp{kg} with regards to \ac{cai}. Before proceeding to that in section~\ref{sec:kg_for_cai} however, this subsection shall briefly summarize the state-of-the-art applications of \acp{kg}, divided by \acp{kg} for knowledge aware applications and \acp{kg} for knowledge acquisition.
%-------------------------------------------
\subsubsection*{\acs{kg}s for knowledge aware applications}
%-------------------------------------------
\acp{kg} in knowledge aware systems aim at an injection of information in order to improve representation learning as defined in subsection~\ref{sub:gnn} \citep{Ji_2022}. In that context, we found \ac{kg} applications for \emph{clustering}, \emph{recommender systems and rule-based learning} by our structured literature review approach.
%-------------------------------------------
\paragraph{Graph clustering for \ac{kg} applications}
In graph clustering, most applications can be divided into \emph{node-clustering}, using distance or similarity as input and \emph{structural clustering}, using the graph topology as input for a clustering algorithm. \\
Beneath the rather established \emph{bi-section k-modes clustering}, proposed by \citet{Schmitz2006}, \citet{Xiao_2021} utilize a multi-view clustering framework in order to overcome the loss of semantics during embedding (see~\ref{sub:kg}), specially for \acp{kg}. %Thereby, the major advantage lies in the generation of semantic representations of \ac{kg} modules within the clustering framework, rendering it a solution to entity retrieval.\\
When it comes to structural clustering, \citet{Elbattah2017} first used the \emph{Louvain} clustering algorithm to differentiate graph vertices into group-forming communities, based on their edge structure, whereafter many authors like \citet{Huang2010LinkPB} built upon it and connected graph clustering to other applications like link prediction based on a clustering coefficient from \ac{kg} topology. Recently, \citet{Tian2014LearningDR} succeded in applying an autoencoder \ac{gnn} for spectral clustering of graph-structured data.

%-------------------------------------------
\paragraph{\acs{kg} recommender systems and rule based learning}
A recommender system is usually a \ac{ml}-based filtering method for providing specific items to a user, based on its predicted preferences \citep{Liu2021}.\\
\acp{kg} can serve as a side information for such systems but require embedding in order to be used as an input for a \ac{ml} model (see~\ref{sub:kg}). Hence, \acp{kge} in the context of recommender systems either construct \acp{kg} with items and their related attributes, referred to as \emph{item graphs} (such as in \citet{GUO202187} or \citep{Wang2018DKNDK}), or directly
builds a so-called \emph{user-item-graph}, where vertices represent users, items, and their respective attributes (such as in \citet{Ai_2018} or \citet{Song2019ExplainableKG}). \\
For a comprehensive survey on other methods for \ac{kg}-based recommender systems, \citet{Liu2021} shall be recommended. \\



\begin{table}[!ht]
\centering
\footnotesize
    \begin{tabular}{p{3cm} p{2cm} p{2cm} p{2cm} p{2cm}}
    \toprule
    \rotatebox{60}{Reference}   & \rotatebox{60}{Representation}    & \rotatebox{60}{Setting}   & \rotatebox{60}{Learning}  & \rotatebox{60}{Comprehensibility} \\
    \toprule
    \citet{Schmitz2006}         & \emph{SB}                         & \emph{KAW}                & \ac{kge}                  & - \\ 
    \bottomrule
    \end{tabular}
    \normalsize
\caption{Characterizations of each scope of the survey}
\label{tab:scop}
\end{table}

%-------------------------------------------
\subsubsection*{\acs{kg}s for knowledge acquisition}
%-------------------------------------------

%-------------------------------------------
\paragraph{\acs{kg} completion}

%-------------------------------------------
\paragraph{Edge extraction}

% grafik für link prediction
%\includegraphics[width=\linewidth]{figures/lp_example.png} \label{fig:query}

==> sections/overview.tex <==
%-------------------------------------------
\section{Overview}\label{sec:ov}
%-------------------------------------------


\acp{kg} are the human- and machine-readable representation of semantically connected data, referred to as knowledge, or knowledge of a certain domain. While several definitions of \acp{kg} were already given in academic literature, such as \citet{paulheimKnowledgeGraphRefinement2016}, \citet{Ehrlinger2016} or \citet{farberWhichKnowledgeGraph09}, this survey aims at an explanation of typical applications of \acp{kg}, which are usually applications already dealing with knowledge, applications designed for the acquisition of knowledge and, most notably, for applications designed for \ac{iml} and \ac{xai}. The following subsection~\ref{sub_hist} will introduce the topic by providing a brief history of \acp{kg}.

%\acp{kg} are the human- and machine-readable representation of semantically linked data referred to as knowledge or knowledge of a particular domain \citep{Hogan_2022}. Semantically linked data is predestinated to explain the complex decision-making of AI methods \citep{ Gaur2021}. This survey aims to be an overview of \acp{cai} methods on \acp{kg}. The following subsection~\ref{sub_hist} will introduce the topic by providing a brief history of \acp{kg}.

%-------------------------------------------
\subsection{A brief history of \acs{kg}s}\label{sub_hist}
%-------Simon locked, 05.04.22-------READY FOR REVIEW---
 Covered in different terminologies, the first \acp{kg} were created as semantic networks as a university project from 1972 to 1980 \citep{Schneider1973CourseMA}. Even though between 1985 and 2007 the idea of a \ac{kg} was applied to different fields, such as human language in \emph{Wordnet}, the success of \acp{kg} skyrocketed when \emph{DBpedia} and \emph{Freebase} were created as general-purpose knowledge bases, which led to the \emph{Google} \ac{kg} in 2012 \citep{singhal_2012}. Since then, a plethora of private companies and academic institutions utilize \acp{kg} for a variety of applications and popular conferences like the \emph{IEEE International Conference on \acs{kg}} were created \citep{Hogan_2022, IEEEKG}. Eventually, most \ac{kg} applications can be found in knowledge-aware systems (e.g. \emph{Wordnet}), or in systems that try to acquire knowledge (e.g. the \emph{Google} \ac{kg}). A burgeoning topic is \ac{cai} and with it \ac{xai} and \ac{iml}, which is why the main body of this paper is structured in three according sections.
 
 %Covered in different terminologies, the first \acp{kg} were created as semantic networks as a university project from 1972 to 1980 \citep{Schneider1973CourseMA}. Even though between 1985 and 2007 the idea of a \ac{kg} was applied to different fields, such as human language in \emph{Wordnet} \citep{Miller1995}, the success of \acp{kg} skyrocketed when \emph{DBpedia} \citep{Auer2007} and \emph{Freebase} \citep{Bollacker2008} were created as general-purpose knowledge bases, which led to the \emph{Google} \ac{kg} in 2012 \citep{singhal_2012}. Since then, a plethora of private companies and academic institutions utilize \acp{kg} for a variety of applications \citep{Hogan_2022}. Eventually, most \ac{kg} applications can be found in knowledge-aware systems (e.g. \emph{Wordnet}), or in systems that try to acquire knowledge (e.g. the \emph{Google} \ac{kg}) \citep{singhal2012google}. A burgeoning topic is \ac{cai} \citep{Futia2020} and with it \ac{xai} and \ac{iml}, which is why the main body of this paper is structured in three according sections.
 
 
 After having sketched a brief history of \acp{kg}, the following subsection~\ref{sub:proc} shall outline the proceeding of this survey.
 
%-------------------------------------------
\subsection{Proceeding of this survey}\label{sub:proc}
%-------Simon locked, 12.3.22-------READY FOR REVIEW---
Following the systematic literature search process of \citet{websterAnalyzingPrepareFuture2002} and \citet{vombrockeReconstructingGiantImportance2009}, we screened for publications on \acp{kg} for knowledge aware systems, knowledge acquisition and predominantly for those with a focus on \ac{iml} and \ac{xai}. 
In order to assure the review of high quality publications, we considered whether journals were listed in ratings, such as the \ac{ais} Senior Scholars' Basket and assessed metrics like the publication power based on Holsapple et al. or the \emph{h}-index \cite{holsapplePublicationPowerApproach2008}, \cite{minasnyCitationsIndexSoil2013}. 
Based on the typology of literature reviews developed by \citet{pareSynthesizingInformationSystems2015}, our survey aims at a narrative approach to describing the state of the art of \acp{kg} for knowledge aware systems, knowledge acquisition, \ac{iml} and \ac{xai}. Eventually, our structured search was conducted using the search strings \emph{"\acf{kg}*" \textbf{AND} "\acf{ml}*" \textbf{OR} "\acf{ai}*"} and \emph{"\acf{kg}*" \textbf{AND} "Interpretable*" \textbf{OR} "Explainable*"} in titles, abstracts, and keywords. We chose
%--- Final number of chosen papers --- 
publications from a total of
%--- Final total number of papers --- 
articles. Following that, we conducted a forward and backward search on the previously selected articles, resulting in the addition of another
%--- Final number of FW/BW papers --- 
articles. Finally, our sample comprised
%--- Final paper count of sample --- 
relevant publications. Figure~\ref{fig:pub_by_year} displays the reviewed publications by year as bars and as cumulative curve. 

%Following the systematic literature search process of \citet{websterAnalyzingPrepareFuture2002} and \citet{vombrockeReconstructingGiantImportance2009}, we screened for publications on \acp{kg} for knowledge aware systems, knowledge acquisition and predominantly for those with a focus on \ac{iml} and \ac{xai}. 
% Based on the typology of literature reviews developed by \citet{pareSynthesizingInformationSystems2015}, our survey aims at a narrative approach to describing the state of the art of \acp{kg} for knowledge aware systems, knowledge acquisition, \ac{iml} and \ac{xai}. Eventually, our structured search was conducted using the search strings \emph{"\acf{kg}*" \textbf{AND} "\acf{ml}*" \textbf{OR} "\acf{ai}*"} and \emph{"\acf{kg}*" \textbf{AND} "Interpretable*" \textbf{OR} "Explainable*" \textbf{OR} "Comprehensible*"} in titles, abstracts, and keywords. 
%We chose
%--- Final number of chosen papers --- 
%publications from a total of
%--- Final total number of papers --- 
%articles. Following that, we conducted a forward and backward search on the previously selected articles, resulting in the addition of another
%--- Final number of FW/BW papers --- 
%articles. Finally, our sample comprised
%--- Final paper count of sample --- 
%relevant publications. Figure~\ref{fig:pub_by_year} displays the reviewed publications by year as bars and as cumulative curve. 

%\begin{table}[!ht]
%    \centering
%        \begin{tabular}{c c c c}
%            \toprule
%            Year & Count of publications & Year & Count of publications  \\
%            \midrule
%            1981 &                 1 & 2013 &                 4 \\
%            2000 &                 1 & 2014 &                 3 \\
%            2002 &                 3 & 2015 &                 7 \\
%            2003 &                 1 & 2016 &                 6 \\
%            2004 &                 2 & 2017 &                 2 \\
%            2008 &                 3 & 2018 &                 2 \\
%            2009 &                 3 & 2019 &                 4 \\
%            2010 &                 1 & 2020 &                11 \\
%            2011 &                 5 & 2021 &                15 \\
%            2012 &                 1 & 2022 &                15 \\
%            \bottomrule
%        \end{tabular}
%    \caption{Reviewed publications by year.}\label{tab:pub_by_year}
%\end{table}

\begin{figure}[!ht]
    \begin{minipage}[b]{0.63\linewidth}
    % TODO: Schrift größer.
      \centering
        \includegraphics[scale=0.21]{figures/akt_pub_by_year.png}
        \caption{Reviewed publications by year.}\label{fig:pub_by_year}
    \end{minipage}
    \begin{minipage}[b]{0.335\linewidth}
    It seems safe to say, that the literature reviewed for the scope of this survey, experienced a skyrocketing amount of publications in the very recent past, while a steady ascent can be postulated since the beginning of the $21^{st}$ century.
    \end{minipage}
\end{figure}

The following subsection~\ref{sub:source} shall detail the proceeding of this survey by describing the literature sources in a more detailed manner.

%-------------------------------------------
\subsection{Sources of this survey}\label{sub:source}
%-------Simon locked, 25.3.22-------READY FOR REVIEW---
Predominantly, journal articles, conference papers, books and book sections were taken into consideration for this survey. However, also a smaller amount of other sources, such as papers on the free distribution service \url{arxiv.com} were regarded, where necessary.\footnote{In few cases, relevant research fields were not covered sufficiently by journal articles, conference papers or books and book sections. In those cases, other sources where taken into account and selected by rampant scores, such as the \emph{h-index}.} Table~\ref{tab:pub_freq} presents the most frequent journals, conferences or publishers of the literature list of this survey.


%Predominantly, journal articles, conference papers, books and book sections were taken into consideration for this survey.  Table~\ref{tab:pub_freq} presents the most frequent journals, conferences or publishers of the literature list of this survey. In order to assure a high quality in selecting sources, we utilized the \emph{Scimago Institutions Rankings}, a ranking of scientific journals and conferences, based on a composite indicator that represents research performance, innovation outputs and societal impact measured by the web visibility of the respective journal or conference \citep{scimagoresearchgroupOECDSCImagoResearch2014, bornmannWhatProportionExcellent2014, bornmannNewExcellenceIndicator2012}. We focused on journals and conference proceedings above rank 150.

\begin{table}[!ht]
    \centering
    \footnotesize
    \begin{tabular}{lrrr}
    \toprule
     Type   &  Book        &  Conference   &  Journal       \\
            &  (section)    &  proceeding  &  article       \\
    Journal, Conference or Publisher                   &                          &                         &                    \\
    \midrule
    Advanced Engineering Informatics                   &                        0 &                       0 &                 6  \\
    Decision Support Systems                           &                        0 &                       0 &                 3  \\
    Expert Systems with Applications                   &                        0 &                       0 &                 6  \\
    IEEE                                               &                        0 &                      25 &                 19 \\
    \bottomrule
    \end{tabular}
    \normalsize
    \caption{Most frequent journals, conferences or publishers.}\label{tab:pub_freq}
\end{table}

In order to assure a high quality in selecting sources, we utilized the \emph{Scimago Institutions Rankings}, a ranking of scientific journals and conferences, based on a composite indicator that represents research performance, innovation outputs and societal impact measured by the web visibility of the respective journal or conference \citep{scimagoresearchgroupOECDSCImagoResearch2014, bornmannWhatProportionExcellent2014, bornmannNewExcellenceIndicator2012}. The ranking lists 1456 conferences and journals and for the scope of this survey, we focused on journals and conference proceedings above rank 150. Table~\ref{tab:ranking} displays the count of publications of selected examples of journals, conferences or publishers by their rank.

\begin{table}[!ht]
    \centering
    \footnotesize
    \begin{tabular}{lrrrr}
    \toprule
    Rank &  7   &  18  &  27  &  37   \\
    Journal, Conference or Publisher                   &      &      &      &       \\
    \midrule
    Advanced Engineering Informatics                   &    0 &    0 &    0 &    6  \\
    Expert Systems with Applications                   &    0 &    0 &    6 &    0  \\
    IEEE Transactions on Neural Networks and Learni... &    3 &    0 &    0 &    0  \\
    Knowledge-Based Systems                            &    0 &    3 &    0 &    0  \\
    \bottomrule
    \end{tabular}
    \normalsize
    \caption{Selected ranking examples.}\label{tab:ranking}
\end{table}

% Figure~\ref{fig:pub_by_type} depicts the count of publications by publication year and type of the publication. It can be stated, that %conference proceedings ran rampant in the recent years, while journal articles in our selection experienced a steady growth overall. Books and %book sections epitomize a rather small fraction of the overall publication types but occur in most of the included years. Assuming conference %proceedings, books and book sections as being published with a certain time lag, the high amount of journal papers in 2022 is worth mentioning.

%\begin{figure}[!ht]
%  \centering
%  \includegraphics[scale=0.3]{figures/akt_pub_by_type.png}
%  \caption{Reviewed publications by type.}\label{fig:pub_by_type}
%\end{figure}

The following subsection~\ref{sub:scop} will outline the actual results as well as the scope of this survey. 

%-------------------------------------------
\subsection{Scope and results of this survey}\label{sub:scop}
%-------Simon locked, 17.3.22-------READY FOR REVIEW---
As stated above, \acp{kg} are not a particular new concept. Especially when it comes to applications of \acp{kg} that include \ac{ml}, academic literature accumulated in the recent past. 

%-------------------------------------------
\subsubsection*{Scope of this survey}
In the following paragraphs, \acp{kg} shall briefly be put into the context of \ac{ml}. Thereby, a simplified, generic pipeline, thus the sequential processing of data shall be stressed, whereby data $x_i$, a \ac{ml} model $\beta$ and a prediction $y_i$ are main building blocks. Figure~\ref{fig:scope} visualizes this simplified, generic \ac{ml} pipeline, as, for instance, elaborated on by \citet{Zhu2020}.

%-------------------------------------------
\paragraph{\acs{kg}s as input for \acs{ml}}
As outlined in subsection~\ref{sub_hist}, \acp{kg} store domain knowledge, which is why there is an increasing interest to use them to improve \ac{ml} models. As will be detailed later, \acp{kg} or \ac{kg} modules can be embedded in order to render their symbolic structure into numerical representations, while also other, purely symbolic methods of using domain knowledge for \ac{ml}, exist \citep{Quinlan1990}.
% es gibt auch ML methoden die rein symbolisch funktionieren. i.e. FOIL https://www.geeksforgeeks.org/first-order-inductive-learner-foil-algorithm/
Thus, within a generic \ac{ml} pipeline, \acp{kg} can be used as an input for any \ac{ml} model $\beta$, which is the setting of most of the academic papers reviewed in this survey. As the following paragraph shall point out, also other settings exist, but shall be left to other scholars.

%-------------------------------------------
\paragraph{\acs{kg}s as output of \acs{ml}}
Apart from being utilized as input for \ac{ml}, \acp{kg} can also be defined as target output representations of an algorithm. Recent progress in computer vision serves as an vivid example, elaborating on techniques that correctly infer relations between detected objects, such as, \emph{window}, \emph{on}, \emph{building} or \emph{building}, \emph{near}, \emph{person} \citep{xuReasoningRCNNUnifyingAdaptive2019}.

% There are other examples, such as in the above-mentioned field of \ac{nlp}, where for instance Dessi et al. elaborated on a \ac{kg} by using \ac{nlp} for an analysis of abstracts of scientific publications \cite{dessiGeneratingKnowledgeGraphs2021}. It has to be stated however that in many cases, \acp{kg} may be generated as output of an \ac{ml} system just to reuse them afterwards  as an input for another \ac{ml} application. Furthermore, it depends on the individual task whether a complete \acp{kg} is produced (see \cite{dessiGeneratingKnowledgeGraphs2021}), or whether single entities and relations are generated and thus added to an existing \ac{kg} (see \cite{dessiGeneratingKnowledgeGraphs2021}). 

%Figure~\ref{fig:scope} displays a simplified, generic \ac{ml} pipeline with \acp{kg} as input or output. Note that the above described ways of using \acp{kg} as input for \ac{ml} (with or without embedding) as well as using \acp{kg} as output for \ac{ml} (with $y_i$ being a complete \ac{kg} $U$ or a module of it respectively).

\begin{figure}[!ht]
    \begin{minipage}[b]{0.63\linewidth}
    % TODO: Schrift größer.
      \centering
    \includegraphics[scale=0.4]{figures/ml_kg_pipeline.png}
    \caption{Simplified, generic \ac{ml} pipeline with \acp{kg} as input or output.}\label{fig:scope}
    \end{minipage}
    \begin{minipage}[b]{0.335\linewidth}
Even though there are further, vivid examples on how \acp{kg} are used as output of \ac{ml}, this survey focuses on \acp{kg} for \ac{cai}, which is why, for the further course of this reading, applications using \acp{kg} are used as output of \ac{ml} shall be left out.
    \end{minipage}
\end{figure}

%ich finde den paragraph sehr gut geschrieben. Es nimmt vieles vorweg, was in \ref{sub:comp} daran gekommen wäre. Ich würde dort erst auf sowas wie uneindeutigkeiten in der definition eingehen. Hier mehr den "Roten Faden" betonen -> KG as Input oder Output, egal wie comprehensiblity is wichtig weil... und darum geht in unserer survey vorallem um cai.

%-------------------------------------------
\paragraph{\acp{kg} for \acs{cai}}
As shall be outlined in subsection~\ref{sub:comp}, \ac{iml} refers to methods that renders the behavior and predictions of \ac{ml} systems understandable to humans \citep{molnarInterpretableMachineLearning2019}. Furthermore, \ac{xai} describes algorithms that are designed with a view to transparency, interpretability and explainability \cite{roscherExplainableMachineLearning2020, murdochDefinitionsMethodsApplications2019, liptonMythosModelInterpretability2018}.
From the repeated mention of the term \emph{interpretable}, or \emph{interpretability} respectively, one can assume that a clear cut distinction between the terms \ac{iml} and \ac{ml} has to be made. In subsection~\ref{sub:comp}, we will come to such a formal distinction, while summarizing both concepts by the notion of \ac{cai}. Amongst others, \citet{tiddiKnowledgeGraphsExplainable2020} elaborated on \acp{kg} for \ac{xai}, while a smaller group of authors refers to interpretability, such as \citet{anelliHowMakeLatent2019} or \citet{gaurSemanticsBlackBoxCan2021}. Hence, a thorough revision of how \acp{kg} are applied for \ac{cai} shall epitomize the crest of the scope of this survey and will be presented in Section~\ref{sec:kg_for_cai}.

%-------------------------------------------
\subsubsection*{Results of this survey}
The publications reviewed in this survey were categorized in the way this survey is structured. According to \citet{websterAnalyzingPrepareFuture2002}, we derived a two-stage literature review matrix based on groups and collections, whereby groups epitomize the first hierarchical level of the two-stage matrix and collections form the second hierarchical level. Table~\ref{tab:scop} displays the generic structure of this matrix, which enables to structure reviewed literature by field of application (\acp{kg} for knowledge aware systems, \acp{kg} for knowledge acquisition and \acp{kg} for \ac{cai}) and method (e.g. \acp{gnn}). A formal presentation of the results of this survey will thus take place in the following sections, which are named after the identified fields of applications, while subsections will outline the rampant methods accordingly.

%\begin{table}[!ht]
%\centering
%\footnotesize
%    \begin{tabular}{ |p{2.9cm}||p{2.7cm}|p{2.7cm}|p{2.7cm}|  }
%     \hline
%     \multicolumn{4}{|c|}{Field of application} \\
%     \hline
%     Publication        & Method 1  & Method $i$    & Method $n$    \\
%    \hline
%     Author, title      &               & x                 &                   \\
%     \hline
%    \end{tabular}
%    \normalsize
%    \caption{Two-stage literature review matrix.}\label{tab:mat}
%\end{table}

\begin{table}[!ht]
\centering
\footnotesize
    \begin{tabular}{l|p{0.8\linewidth}}
    \toprule
    Scope                  & Characterization \\
    \toprule
    Representation      & Symbolic (\emph{SB}), Sub-symbolic (\emph{SSB}), Neuro-symbolic(\emph{NSB}). \\ 
    \midrule
    Setting             & Knowledge-aware-system (\emph{KAW}), \\
                        & Knowledge-acquisition-system (\emph{KAQ}). \\
    \midrule
    Learning            & Factorization-machine \emph{FM}, Transnational \emph{T}, Rule-based (\emph{RB}),  \\
                        & Tree-based (\emph{TB}), \acs{ann} (\emph{NN}), Others (\emph{O}).  \\
    \midrule
    Task                & Link-prediction \emph{LP}, Node-prediction \emph{NP}, Node-classification \emph{NC}, \\ 
                        & Graph-classification \emph{GC}, Clustering \emph{C}, Recommendation \emph{R}.  \\
    \midrule                   
    Comprehensibility   & \acs{iml} (\emph{\ac{iml}}), \\
                        & \acs{xai} (\emph{\ac{xai}}).\\
    \bottomrule
    \end{tabular}
    \normalsize
\caption{Characterizations of each scope of the survey}
\label{tab:scop}
\end{table}

Since the scope of this review is limited, the full literature review matrix shall not be depicted here, but provided as appendix. Hence, the following section introduces pivotal methodology and definitions.



==> sections_short/00_Answer_to_the_reviewer.tex <==
% Habe mich hier an dem Revision Report bei IEE TVCG von Joscha orientiert. 

\section*{Revision Report}

We like to thank the reviewers for their very helpful comments and the chance to submit our paper to the Journal of Web Semantics with a major revision.

We rigorously revised the survey regarding how the findings are served. This includes updated explanations of key terms, like a formal definition of XAI and IML, in addition to the previously provided definition by examples. We also improved the communication of groups of methods by updating the descriptions of the methods and the novel Tables 4 and 5. 
Additionally, we significantly improved the cited papers' description by adding vital information and describing previously cited but undescribed papers. Finally, the paper was carefully checked regarding the formulations (including section names), grammar, and typos. The detailed comments of the reviewers and the corresponding answers and changes are listed below, organized by topic.

We are now confident that our paper adequately addresses the reviewers' comments and will make an excellent addition to the Journal of Web Semantics. We thank all reviewers again for their valuable comments and time, and acknowledge that they resulted in notable improvements to our paper. The following sections explain how their feedback was included in the paper. In sum, the paper has significantly improved in this major revision, and we believe our contributions are now even clearer and stronger. We look forward very much to the reviewer's comments. \\

Best regards, \\
Simon Schramm, Christoph Wehner, and Ute Schmid

%ANMERKUNG: ich habe die reviews gegliedert. Wir können jetzt unsere antworten unter die paragraphen schreiben. Am aufbau darfst du gerne rumdoktern. Wir sollten uns aber nicht verkünsteln.
% Ich finde, wir sollten den revision report einspaltig formatieren. 

\section*{On the Distinction of CAI, XAI, and IML}
\paragraph{Adding some illustration to show the distinction between XAI, IML and CAI in the introductory section would make the distinction more understandable} \mbox{}\\
Thank you for this remark. We have added Figure 1 (p.1) to the introduction. Figure 1 illustrates the distinction between XAI, IMl, and CAI.

\paragraph{The difference of XAI and IML is first explained on page 2 in the left column. This explanation is not well done as it introduces two papers which are probably not known to most readers. They might be perfect examples, however, at the end one understands the difference by the explanation in the text and not by looking at the papers. Its not good to start the whole thing with a reference to two papers, which might not be known to most readers. If it is done this way, then the context of the paper needs to be explained in more details … I personally believe that it is better to explain the difference not with an example but with an explanation on the abstract level} \mbox{}\\ 
We believe you are right. Previously, the reader was introduced to XAI, IML, and CAI via example papers. 
We updated Section 1 with an abstract introduction to XAI, IML, and CAI (p.1). Additionally, we strengthened the support for our distinction with additional citations. 

\paragraph{On Page 5 you write: "(1) The CAI model is supposed to justify its output and show if the output is ethical in a predominant moral system". This sentence mixes two things in an inappropriate way. The main point here is that a CAI model is supposed to justify its output. This can than be used, for example, to show if the output is ethical in a predominant moral system. However, this is just one possible application. The way how the sentences is phrased is sound as if the ethical check belongs to the core aspect of a CAI model} \mbox{}\\
Thank you for pointing this out. The way the sentence was phrased indeed inappropriately mixes two things. We rephrased the sentence such that it now states clearly that this is just one possible exemplary application (p.5). 

\section*{Scope of the Survey}
\paragraph{The paper is concerned with comprehensible Artificial Intelligence on Knowledge Graphs. One would expect that it deals with any kind of AI algorithms that are somehow concerned with knowledge graphs. This is a bit weird as this covers very different algorithms and especially also very different purposes and goals. It is a bit unclear why it makes sense to choose the use of knowledge graphs as the aspect that these different methods have somehow in common. In the abstract the authors refer to "Knowledge Graph (KG) methods" and later they talk about AI or machine learning "on knowledge graphs". To me it is unclear what kind of methods this covers and what not} \mbox{}\\
We would like to thank you for pointing at this weakness in our argumentation. We sharpened the description of the scope of our survey in Section 1.3 (p.3,4), outlining that we consistently searched for literature that takes \acp{kg} as an input. KGs as target output representations of an \ac{ai} model cannot render the model interpretable, nor can they themselves fulfill the requirements of \ac{xai}. This is why we made this choice and illustrated it in Figure 3. Furthermore, we refer to the term \ac{ai}, since we take both methods that learn themselves as well as post-hoc explanations without self-learning methods.

\paragraph{The explanation of the symbolic representation of KGs is misleading. After reading that section it remains unclear if description logics is one way or the only way to represent a graph in a symbolic way. Moreover, it is in also misleading as it uses a vocabulary (here classes) which is not even part of the graph. It would have been more correct to say that the definition of the graph from the previous section is based or uses a symbolic representation. The important point here is that the algorithms remain in that representation and do not need to map this representation to another representation. Thus, I would start with the sub symbolic representation and explain afterwards that a symbolic representation is just the absence of a mapping to the sub symbolic level} \mbox{}\\
Thank you for pointing out that the explanation of the symbolic representation of KGs is misleading. We carefully considered your suggestions on how to restructure Subsection 2.3.1 (p. 6). We closely stick to your suggestions. We now start by describing the sub-symbolic representation and, afterwards, the symbolic representation. Additionally, we highlight that the "default"-definition of a KG is symbolic.

\paragraph{The distinction in 2.2.2. is unclear. It seems to be based on the difference between induction and deduction. If this is the core element of the distinction than induction and deduction should be explained. And what about transductive predictions? To which category do they belong? - The distinction becomes even more problematic when you continue with Section 2.2.3. Here recommendation is KAW, while link prediction is said to be KAQ. However, recommendation tasks can be phrased rather naturally as link prediction tasks. See for example (1). Given that, the KAW and KAQ distinction makes no sense, and I would recommend supressing it completely from the paper} \mbox{}\\
We agree with your remark and would like to thank you for this valuable contribution to the quality of our survey. For us, link prediction was an example of knowledge acquisition, since new knowledge is created, here in the form of the prediction of a triplet that did not exist in the Knowledge Graph before. However, after an assessment of the recommended resource \citet{Sola2022}, we decided to remove this distinction from our taxonomy and followed your recommendation.

%[1] Diana Sola, Christian Meilicke, Han van der Aa & Heiner Stuckenschmidt: On the Use of Knowledge Graph Completion Methods for Activity Recommendation in Business Process Modeling. BPM Workshops 2021.

\paragraph{I'm a bit puzzled with 2.2.4 where the different methods are called Optimization methods. I doubt that it makes sense to call the method used in a rule learning approach optimization method. Why not just change from "optimization methods" to just calling them "methods". I'm fully aware that quite often these methods are optimization methods, however, sometimes they are not optimization methods} \mbox{}\\
We internally discussed your suggestion. We concluded that your argument is valid. The phrase "optimization" does not apply to all methods we aim to include. We want to suggest  "Foundational methods" (i.e. Foundation) instead. The methods described in Section 2.3.3 are the assessed papers' foundational machine learning methods/techniques/approaches. In other words, Section 2.3.3 describes the methods that build the methodological bases of the assessed papers.

\paragraph{One of the most important contributions of the paper is a bit hidden, as it does not appear in Table 4. This is the distinction of they different approaches to explain a complex model in Section 3.1 and 3.2. E.g. Using rules as explanation, using surrogate methods, using graph generation ect. However, this different methods could be explained in more details, also pointing to overlaps between them in more details. For example: Why is a model that learns rules to solve a task and to explain the solution not also a surrogate methods. It falls 100\% under the definition "Approximating the predictions of a black-box model by deploying a more simple yet interpretable model is referred to as a surrogate method". It should be explained why it is not like this.
I recommend splitting Table 4 into two larger tables, one for IML and one for XAI. Then I would replace the last column by a column that informs on the specific approach. And I do not see any useful information in the distinction between KAW and KAQ, which given more than the Task column. This I would also remove this column and completely remove this dimension} \mbox{}\\
Thank you for this valuable contribution. We followed your advice and split table 4 into two tables, one for IML (Table 4 p.11) and one for XAI (Table 5 p.16). Furthermore, we added a column called "Lines of research", which provides additional information about the respective line of research from our taxonomy as well as a brief description of the main contributions of one or more papers.
% Table 4 aufteilen und Table 2 ergänzen inkl. Verweis auf "Lines of research" als contribution Simon \\
% Spalte "Line of research" befüllen + Beschreibung in Intro von Kap. 3. Beide \\
% Hinweis: Bei mehreren Quellen bauen die Paper auf einander auf. \\
% Kursiv-Schreibung bei Acro-Package checken. Eigennamen, Abkürzungen nicht kursiv. \\
% Trennline nach XGNN

\section*{Assessed Literature}

\paragraph{In 3.1.1. the authors claim that rule-based approaches suffer from scalability. This is wrong. See for example the results in (2). Here the authors compare state of the art embedding based approaches to AnyBURL, one of the rule-based approaches that you mention, including also some runtime results. According to these results AnyBURL is faster. Three references are mentioned to support these claims (73,74,75). These are from 1995 to 2011! In a literature review I would expect a better foundation for such a claim. In this case there is, even more, some evidence that the claim is wrong} \mbox{}\\

Thank you for this valuable feedback. Indeed, our claim regarding scalability was wrong. We corrected the wrong claim and included Rossi et. Al. \cite{rossi2021} as a citation. We rephrased all appearances (p.2,6,8) of the claim such that the survey now clearly states that scalability was an issue of early ILP approaches on KGs such as \citep{Cohen1995,Svatek2006,Lao2011}, and successful research efforts led to an improvement on this issue such that recent approaches such as AnyBURL demonstrate state-of-the-art performance. 

\paragraph{The sentence "Gad-Elrab et al. address the issue of embeddings being latent and without great contribution to the explainability of a prediction" is not well written. I had to read it several times to understand that it is not saying that Gad-Elrab wrote a paper without great contribution} \mbox{}\\
Thank you for pointing out this inaccuracy. We rephrased the sentence for better understanding.
% Umformulieren Simon \\

\paragraph{The survey can be a bit longer, and I think it would make sense to give a short summary for all papers you listed in Table 4. Some of them are not explained at all. At least they should all be mentioned in the main text somehow} \mbox{}\\
We assessed the length of the descriptions of the papers included in the survey and added significant content, where applicable. Additionally, we added a description of all previously not described papers (e.g. \citep{Hou2021}, \citep{Hou2021}, ...). Finally, we added Figures 7, 8 and 9 from the researched papers, where helpful, and included a description for better understanding of the content accordingly. 
% Beschreibungen der Paper in langversion checken. Beide.

\section*{Others}
\paragraph{Figure 3 should be enlarged, especially the text is too small} \mbox{}\\
Figure 3 from the initial submission is now Figure 1, whereby the text size was enlarged as much as possible given the figure content.
% Anpassen wie gewünscht Simon

\paragraph{The titles of the sections are not well chosen. An example can be found in the Title of Section 2. This title is far to long. However, that is not the main problem. The main problem is that Section 2 simply introduces the taxonomy used in this paper, which is shown in Table 2, and it takes some time to see this, as its not explicitly said and the titles are so long. Moreover, each subsection of 2.2 corresponds to one row in the Table, while 2.1 corresponds to the last row in the Table. It would be much easier to see this if the Section s would simply be called "Setting", "Task", "Optimization", instead of e.g. "Optimization of Comprehensible Artificial Intelligence on Knowledge Graphs". The whole paper is about Artificial Intelligence on Knowledge Graphs and there is no need to repeat it in each Section Title} \mbox{}\\
We would like to thank you for that constructive remark. We followed your suggestion and shortened the titles in Section 2. We also made some changes in the wording, so that the titles are precise, and the style is consistent. 
% Anpassen wie gewünscht Simon \\
% Überschriften angepasst, Aufbau des Kapitels 2.2.x an Table anzupassen --> Foundational Methods -> Foundation

\paragraph{Although this survey paper has fairly chosen the existing papers on CAI, adding some more relevant papers on both XAI and IML in relevance to CAI would make this survey more comprehensive} \mbox{}\\
We would like to thank you for your remark. In case "on both XAI and IML in relevance to CAI" refers to the definition of CAI and the differentiation of XAI and IML as subordinate notions, we reassessed our abstract/formal definition in the text. We would like to stress the example we put forward already in Section 1, describing \emph{TEM} (\citet{Wang2018}) and \emph{RelEx} (\citet{Zhang2021}) as vivid representatives of IML (TEM) and XAI (RelEx), due to their specific characteristics. Also, we would also like to point at Figure 1, which visualizes the concept. Eventually, we are convinced that the most relevant papers for the definition of CAI are mentioned in the text and hope you can agree. \\
In case "on both XAI and IML in relevance to CAI" refers to the total amount of papers that deal with CAI on KGs in the survey, we reassessed the papers included and came to the conclusion that the most important works for CAI on KGs are included. However, we decided to enlarge the description of the existing papers described in our survey and thus added significant content to Section 3. \\
Since we were not completely sure which of the above-cases was meant, we elaborated on both. Additionally, we reached out to the Journal in order to clarify this question. We hope that our enhancements can live up to what was meant by your remark.
% we reached out to the Journal recently. 
% --> Fragen: Mehr Paper zur Unterscheidung zwischen XAI und IML in Verbindung mit CAI - oder mehr Paper in der Survey? Simon \\
% --> Per E-Mail nachfragen. \\




